A New Conjecture on Hardness of Low-Degree 2-CSP's with Implications to Hardness of Densest $k$-Subgraph and Other Problems

We propose a new conjecture on hardness of low-degree $2$-CSP's, and show that new hardness of approximation results for Densest $k$-Subgraph and several other problems, including a graph partitioning problem, and a variation of the Graph Crossing Number problem, follow from this conjecture. The conjecture can be viewed as occupying a middle ground between the $d$-to-$1$ conjecture, and hardness results for $2$-CSP's that can be obtained via standard techniques, such as Parallel Repetition combined with standard $2$-prover protocols for the 3SAT problem. We hope that this work will motivate further exploration of hardness of $2$-CSP's in the regimes arising from the conjecture. We believe that a positive resolution of the conjecture will provide a good starting point for further hardness of approximation proofs. Another contribution of our work is proving that the problems that we consider are roughly equivalent from the approximation perspective. Some of these problems arose in previous work, from which it appeared that they may be related to each other. We formalize this relationship in this work.

==> DkS-inner-thm-backup.tex <==
\iffalse
\begin{theorem}\label{thm: partition or solution for no instance}
	Assume that there exists an efficient $\alpha(N)$-approximation algorithm $\aset$ for the \DS problem, where $N$ is the number of vertices in the input graph. Then there is an efficient randomized algorithm, that, given an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP and a parameter $n$, so that $\size(\iset)\leq n$, and  $\iset$ is a $d(n)$-to-$d(n)$ instance of 2-CSP, together with parameters $\gamma,\beta\geq 1$, with $\beta \geq 2^{23}\gamma^3(\alpha(n))^3(\log n)^{12}$, does one of the following:
	
	\begin{itemize}
		\item either correctly establishes that graph $H(\iset)$ is $\beta^3$-good; or
		
		\item computes a $\gamma$-bad set $\cset'\subseteq \cset$ of constraints, with $|\cset'|\geq \frac{|\cset|}{8\log^2n}$; or
		\item  computes a subgraph $H'=(X',Y',E')$ of $H(\iset)$, for which the following hold:
		\begin{itemize}
			\item $|X'|\leq \frac{2d(n)\cdot |X|}{\beta}$;
			\item $|Y'|\leq \frac{2d(n)\cdot |Y|}{\beta}$; and
			\item $|E'|\geq \frac{\vol_H(X'\cup Y')}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$.
		\end{itemize}
	\end{itemize} 
\end{theorem}
\fi



\subsection{Proof of \Cref{thm: partition or solution for no instance}}
\label{subsec: proof of inner thm for DkS}

For convenience, we denote $H=H(\iset)$. If $|E(H)|\leq \beta^3$, then  graph $H$ is $\beta^3$-good, since we can compute an assignment to the variables of $X\cup Y$ that satisfies at least one constraint of $\cset$. Therefore, we assume from now on that $|E(H)|>\beta^3$. We can also assume that graph $H$ is connected, as isolated vertices of $H$ correspond to variables that do not participate in any constraints, and can be discarded.


%\mynote{will need $\beta'\geq \alpha^2\log^8A$}
The proof consists of four steps. In the first step, in order to simplify the proof, we will regularize graph $H$, by computing a ``nice'' subgraph $\tH\subseteq H$. In the second step, we will define an \emph{assignment graph} associated with $\tilde H$, and we will use it in order to obtain an instance of \DS, to which algorithm $\aset$ will then be applied. In the last two steps, we will use the outcome of algorithm $\aset$ in order to either correctly establish that graph $H$ is $\beta'$-good, or to compute a $\gamma$-bad subset of constraints, or a subgraph $H'$ of $H$ as required. We now describe each of the three steps in turn.



\subsubsection{Step 1: Regularization}

In this step we will compute a subgraph $\tilde H$ of $H$ that has a convenient structure. We refer to graphs with such structure as \emph{nice subgraphs} of $H$, and define them next.

	
\begin{definition}[Nice Subgraph of $H$]
		Let $\tilde H=(\tilde X,\tilde Y,\tilde E)$ be a subgraph of $H$, and let $d_1,d_2\geq 1$ be parameters. We say that $\tilde H$ is a $(d_1,d_2)$-nice subgraph of $H$, if the following hold:
		\begin{itemize}
			\item For every vertex $x\in \tilde X$, $d_1\leq \deg_{H}(x)< 2d_1$; 
			
			\item For every vertex $y\in \tilde Y$, $d_2\leq \deg_{H}(y)< 8d_2\log n$ and
			$d_2\leq \deg_{\tilde H}(y)< 2d_2$; and
			
			\item $|\tilde E|\geq \frac{d_1}{4\log n}\cdot |\tilde X|$.
		
		\end{itemize}
		We say that $\tilde H$ is a \emph{nice} subgraph of $H'$ if it is a $(d_1,d_2)$-nice subgraph of $H$ for any pair $d_1,d_2\geq 1$ of parameters.
	\end{definition}
	
	
	The first step of our algorithm is summarized in the following claim, that allows us to compute a nice subgraph $\tilde H$ of $H$ that contains many edges of $H$.
	
	\begin{claim}\label{claim: regularizing constraint graph}
		There is an efficient algorithm, that computes parameters $d_1,d_2>1$, and a subgraph $\tilde H$ of $H$, such that $\tilde H$ is a $(d_1,d_2)$-nice subgraph of $H$, and  $|E(\tilde H)|\geq \frac{|E(H)|}{8\log^2n}$.
	\end{claim}
	

	\begin{proof}
		The proof uses standard reglarization techniques, and consists of three steps. Denote $H=(X,Y,E)$. 
		
		In the first step, we partition the vertices of $X$ into  groups $S_0,\ldots,S_q$, for $q=\ceil{\log n}$, where for all $0\leq i\leq q$, $S_i=\set{x\in X\mid 2^i\leq \deg_{H}(x)<2^{i+1}}$.
		We also partition the set $E$ of edges into subsets $E_0,\ldots,E_q$, where for all $0\leq i\leq q$, set $E_i$ contains all edges $e\in E$ that are incident to vertices of $S_i$. Clearly, there is an index $0\leq i^*\leq q$, with $|E_{i^*}|\geq \frac{|E(H)|}{2\log n}$. We let $\tilde X=S_{i^*}$, and we let $H_1$ be the graph whose vertex set is $\tilde X\cup Y$, and edge set is $E_{i^*}$. We also define $d_1=2^{i^*}$. Clearly, for every vertex $x\in \tilde X$, $d_1\leq \deg_H(x)<2d_1$. This completes the first regularization step.
%	Notice that for every vertex $x\in \tilde X$, $\deg_{H_1}(x)<2d_1$ also holds.
	
		
	%	; in this case, all edges incident to $x$ are also said to belong to group $q$. Clearly, there is some group $q$ that contains at least $|E(H')|/\log N$ edges. We denote $d_1=2^q$. We then discard from $H'$ all vertices of $X'$, except those lying in group $q$. Let $\tilde H$ be the resulting graph. Then for every vertex $x\in V(\tilde H)\cap X'$, $d_1\leq \deg_{\tilde H}(x)<2d_1$, and $|E(\tilde H)|\geq |E(H')|/\log N$. In the next step, we will discard some vertices from $Y'$, to obtain the final graph $\tilde H$. Clearly, for every vertex $x\in V(\tilde H)\cap X'$, $\deg_{\tilde H}(x)<2d_1$ will continue to hold.
		
		
We now proceed to describe our second step, in which we consider the vertices of $y\in Y$ one by one. We say that a vertex $y\in Y$ is \emph{bad}, if $\deg_{H_1}(y)<\frac{\deg_{H}(y)}{4\log n}$. Let $Y''\subseteq Y$ be the set of all bad vertices, and let $Y'=Y\setminus Y''$ be the set of all remaining vertices of $Y$, that we refer to as \emph{good vertices}.
We use the following observation.


\begin{observation}\label{obs: few edges incident to bad vertices}
	$\sum_{y\in Y''}\deg_{H_1}(y)\leq \frac{|E(H_1)|}{2}$.
\end{observation}
\begin{proof}
	Since, for every bad vertex $y$, $\deg_{H_1}(y)<\frac{\deg_{H}(y)}{4\log n}$, we get that:
	
	\[\sum_{y\in Y''}\deg_{H_1}(y)<\sum_{y\in Y''}\frac{\deg_{H}(y)}{4\log n}\leq \frac{|E(H)|}{4\log n}. \]
	
	Since, as observed above, $|E(H_1)|\geq \frac{|E(H)|}{2\log n}$, the observation follows.
\end{proof}

We let $H_2$ be a graph that is obtained from $H_1$, by discarding the vertices of $Y''$ from it. Therefore, $V(H_2)=\tilde X\cup Y'$. Additionally, from \Cref{obs: few edges incident to bad vertices}, $|E(H_2)|\geq \frac{|E(H_1)|}{2}\geq \frac{|E(H)|}{4\log n}$.

		
Lastly, in our third step, we perform a geometric grouping of the vertices of $Y'$ by their degree in $H_2$. 
Specifically, we let $r=\ceil{\log n}$, and we partition the vertices of $Y'$ into sets $S'_0,\ldots,S'_r$, where for $0\leq j\leq r$, $S'_j=\set{y\in Y'\mid 2^j\leq \deg_{H_2}(y)<2^{j+1}}$.
As before, we also partition the set $E(H_2)$ of edges into subsets $E'_0,\ldots,E'_r$, where for $0\leq j\leq r$ set $E'_j$ contains all edges $e\in E(H_2)$ that are incident to the vertices of $S'_j$. As before, there must be an index $0\leq j^*\leq r$ with $|E'_{j^*}|\geq \frac{|E(H_2)|}{2\log n}\geq \frac{|E(H)|}{8\log^2n}$. We set $\tilde Y=S'_{j^*}$, $d_2=2^{j^*}$, and we let $\tilde H$ be the graph whose vertex set is $\tilde X\cup \tilde Y$, and edge set is $E'_{j^*}$. We now verify that this graph has all required properties.

First, as observed already, for every vertex $x\in \tilde X$, $d_1\leq \deg_H(x)<2d_1$. Let $\tilde E=E(\tilde H)$. As observed already, $|\tilde E|\geq \frac{|E(H)|}{8\log^2n}$. Moreover, since, for every vertex $x\in \tilde X$, $\deg_{H_1}(x)=\deg_H(x)\geq d_1$, we get that $|E(H_1)|\geq d_1\cdot |\tilde X|$, and so $|\tilde E|\geq \frac{|E(H_2)|}{2\log n}\geq \frac{|E(H_1)|}{4\log n}\geq \frac{d_1}{4\log n}\cdot |\tilde X|$.

Consider now some vertex $y\in \tilde Y$. From the definition of graph $\tilde H$, it is immediate to verify that $\deg_{\tilde H}(y)=\deg_{H_2}(y)$. Therefore, $d_2\leq \deg_{\tilde H}(y)\leq 2d_2$. 
Clearly, $\deg_H(y)\geq \deg_{\tilde H}(y)\geq d_2$. Lastly, since vertex $y$ is good, we get that:

\[\deg_{\tilde H}(y)=\deg_{H_2}(y)=\deg_{H_1}(y)\geq \frac{\deg_H(y)}{4\log n}.  \]

Since $\deg_{\tilde H}(y)\leq 2d_2$, we get that $\deg_H(y)\leq (4\log n)\deg_{\tilde H}(y)<8d_2\log n$. We conclude that
$d_2\leq \deg_{H}(y)< 8d_2\log n$.
\end{proof}

	
	
	
\subsubsection{Step 2: Assignment Graph and Reduction to \DS}

Recall that we have defined, in the first step, a subgraph $\tilde H=(\tilde X,\tilde Y,\tilde E)$ of the graph $H=H(\iset)$. Since every edge of $H$ is associated with a distinct constraint in $\cset$, we can define a collection $\tilde \cset\subseteq \cset$ of constraints corresponding to the edges of $\tilde H$: $\tilde \cset=\set{C\in \cset\mid e_C\in \tilde E}$. 


Next, we define a bipartite graph $G=(U,V,\hat E)$, called \emph{assignment graph}, that is associated with graph $\tilde H$.
For every variable  $z\in \tilde X\cup \tilde Y$, we define a set $R(z)=\set{v(z,a)\mid 1\leq a\leq A}$ of vertices that represent the possible assignments to variable $z$. 
%Similarly, for every variable $y\in \tilde Y$, we define a set
%$R(y)=\set{v(y,a')\mid 1\leq a\leq A'}$ of vertices representing the assignments to $y$. For a variable $z\in \tilde X\cup \tilde Y$, we refer to the set $R(z)$ of vertices as the \emph{cloud of $z$}. 
We then set $U=\bigcup_{x\in \tilde X}R(x)$, and $V=\bigcup_{y\in \tilde Y}R(y)$. The set of vertices of $G$ is defined to be $U\cup V$.


In order to define the edges, 
	consider any constraint $C=(x,y)\in \tilde \cset$. We define a set $E(C)$ of at most $d(n)\cdot A$ edges corresponding to $C$, as follows: we add an edge between vertex $v(x,a)$ and vertex $v(y,a')$ to $E(C)$ if assignments $a$ to $x$ and $a'$ to $y$ satisfy the constraint $C$. Since instance $\iset$ is a $d(n)$-to-$d(n)$ instance of Bipartite 2-CSP, every vertex of $R(x)\cup R(y)$ is incident to at most $d(n)$ edges of $E(C)$.
	We then let $E(G)=\bigcup_{C\in \tilde \cset}E(C)$.
	

Let $k_1=|\tilde X|$ and $k_2=|\tilde Y|$. We can then view graph $G$, together with parameters $k_1$ and $k_2$ as an instance of the  \DS problem, $\pdks(G, k_1,k_2)$. Notice that $|V(G)|\leq |\tilde \cset|\cdot A^2\leq |\cset|\cdot A^2\leq \size(\iset)\leq n$. We apply Algorithm $\aset$ to instance $\pdks(G, k_1,k_2)$ of \DS, and we let $S$ be the solution that the algorithm returns. Denote $G'=G[S]$, so the value of the solution is $|E(G')|$. Assume first that $|E(G')|<\frac{|\tilde \cset|}{\gamma\cdot \alpha(n)}$. We use the following observation to show that, in this case, the set $\tilde \cset$ of constraints in $\gamma$-bad.

\begin{observation}\label{obs: bad se of constraint}
	If the set $\tilde \cset$ of constraints is not $\gamma$-bad, then the value of the optimal solution to instance $\pdks(G, k_1,k_2)$ of \DS is at least 
\end{observation}	
\begin{proof}	
Assume that the set $\tilde \cset$ of constraints is not $\gamma$-bad. Then there is an assignment $f$ to variables of $\tilde X\cup \tilde Y$ that satisfies more than $\frac{|\tilde \cset|}{\gamma}$ constraints of $\tilde \cset$. For each variable $z\in \tilde X\cup \tilde Y$, we denote the corresponding assignment by $f(z)$. Let $S'$ be the set of vertices of $G$ that contains, for every variable $x\in \tilde X$, vertex $v(x,f(x))$, and for every variable $y\in \tilde Y$, vertex $v(y,f(y))$. Then $S'$ is a valid solution to instance $\pdks(G, k_1,k_2)$ of \DS. Moreover, for every constraint $C\in \tilde \cset$ that is satisfied by the assignment $f$, an edge of $E(C)$ must be contained in $G[S']$. Therefore, the value of solution $S'$ is at least $\frac{|\tilde \cset|}{\gamma}$. 
\end{proof}

From \Cref{obs: bad se of constraint}, if the set $\tilde \cset$ of constraints is not $\gamma$-bad, then algorithm $\aset$ must have returned a solution whose value is at least $\frac{|\tilde \cset|}{\gamma\cdot \alpha(n)}$. Therefore, if the value of the solution $S$ that the algorithm returns is less than $\frac{|\tilde \cset|}{\gamma\cdot \alpha(n)}$, then we terminate the algorithm, and return $\tilde \cset$ as a $\gamma$-bad set of constraints. Recall that, from \Cref{claim: regularizing constraint graph}, $|\tilde \cset|=|E(\tilde H)|\geq \frac{|E(H)|}{8\log^2n}=\frac{|\cset|}{8\log^2n}$.
From now on we assume that the value of the soution $S$ is at least $\frac{|\tilde \cset|}{\gamma\cdot \alpha(n)}$.
We will use the set $S$ of vertices of $G$, in order to either correctly certify that graph $H$ is $\beta$-good, or to compute a subgraph $H'\subseteq H$ with the required properties. It will be convenient for us to further regularize graph $G'$, which we do in the next step.



\subsubsection{Step 3: Further Regularization}
It would be convenient for us to further regularize graph $G'$, by computing a subgraph $G''\subseteq G'$, with $|E(G'')|$ roughly comparable to $|E(G')|$, that has the following additional properties. First, for all  variables $x\in \tilde X$ with $R(x)\cap V(G'')\neq \emptyset$, the cardinalities of the sets $R(x)\cap V(G'')$ of vertices are roughly equal to each other (to within factor $2$). Similarly, for all  variables $y\in \tilde Y$ with $R(y)\cap V(G'')\neq \emptyset$, the cardinalities of the sets $R(y)\cap V(G'')$ of vertices are roughly equal to each other. Lastly, for all constraints $C\in \tilde \cset$ with $E(C)\cap E(G'')\neq \emptyset$, 
the cardinailities of the sets $E(C)\cap E(G'')$ of edges are roughly equal to each other. In this step, we compute a subgraph $G''\subseteq G'$ with all these properties. The algorithm is summarized in the following claim.
	
\begin{claim}\label{claim: regularization}
There is an efficient algorithm to compute a subgraph $G''\subseteq G'$, subsets $X^*\subseteq \tilde X$, $Y^*\subseteq \tilde Y$ of variables, a subset $\cset^*\subseteq \tilde \cset$ of constraints, and integers $q,q',r\geq 1$, such that, if we denote, for every variable $z\in X^*\cup Y^*$,  $R'(z)= R(z)\cap V(G'')$, and for every constraint $C\in \cset^*$, $E'(C)= E(C)\cap E(G'')$, then the following hold:
		
\begin{itemize}
\item for every variable $x\in X^*$, $2^q\leq |R'(x)|< 2^{q+1}$, and for $x\not\in X^*$, $R(x)\cap V(G'')=\emptyset$;
\item for every variable $y\in Y^*$, $2^{q'}\leq |R'(y)|< 2^{q'+1}$, and for $y\not\in Y^*$, $R(y)\cap V(G'')=\emptyset$;
\item for every constraint $C\in \cset^*$, $2^r\leq |E'(C)|<2^{r+1}$, and for $C\not\in \cset^*$, $E(C)\cap E(G'')=\emptyset$;  and
			%		\item if $C=(x,y)\in E^*$, and $e=((x,a),(y,a'))\in E'(C)$, then $(x,a)\in S'(x)$ and $(y,a')\in S'(y)$; and
\item $|\cset^*|\geq \frac{|\tilde \cset|}{2^{r+4}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$.
\end{itemize}
\end{claim}
	
\begin{proof}
The proof follows a standard regularization process. Let $E^0=E(G')$, so that $|E^0|\geq \frac{|\tilde \cset|}{\gamma\cdot \alpha(n)}$.
		

Our first step regularizes the variables of $\tilde X$. We group the variables of $\tilde X$ into sets $J_0,J_1,\ldots,J_{\ceil{\log A}}$. For all $0\leq i\leq \ceil{\log A}$, we let $J_i=\set{x\in \tilde X\mid 2^i\leq |R(x)\cap V(G')|<2^{i+1}}$.
Note that, if $R(x)\cap V(G')=\emptyset$, then variable $x$ does not belong to any of the groups that we have defined. We also partition the edges of $E^0$ into groups $E_0,E_1,\ldots,E_{\ceil{\log A}}$, where for all $0\leq i\leq \ceil{\log A}$, group $E_i$ contains all edges $e\in E^0$ that are incident to the vertices of $\bigcup_{x\in J_i}(R(x)\cap V(G'))$. It is easy to verify that $(E_0,\ldots,E_{\ceil{\log A}})$ is indeed a partition of the set $E^0$ of edges. Therefore, there is an index $0\leq q\leq \ceil{\log A}$ with $|E_q|\geq \frac{|E^0|}{2\log A}\geq \frac{|E^0|}{2\log n}$. We then set $X^*=J_q$. For each such variable $x\in X^*$, we let $R'(x)=R(x)\cap V(G')$, and for each variable $x\in \tilde X\setminus X^*$, we set $R'(x)=\emptyset$. We also let $E^1=E_q$. From the above discussion,  $|E^1|\geq \frac{|E^0|}{2\log n}$, and, for every variable $x\in X^*$, $2^q\leq |R'(x)|<2^{q+1}$. Note that all edges of $E^1$ are incident to vertices of $\bigcup_{x\in X^*}R'(x)$.
		

Our second step is to regularize the variables of $\tilde Y$, exactly as before. 
We group the variables of $\tilde Y$ into sets $J'_0,J'_1,\ldots,J'_{\ceil{\log A}}$. For all $0\leq i'\leq \ceil{\log A}$, we let $J'_{i'}=\set{y\in \tilde Y\mid 2^{i'}\leq |R(x)\cap V(G')|<2^{i'+1}}$.
As before, if $R(y)\cap V(G')=\emptyset$, then variable $y$ does not belong to any of the sets that we have defined. We also partition the edges of $E^1$ into sets $E'_0,E'_1,\ldots,E'_{\ceil{\log A}}$, where for all $0\leq i'\leq \ceil{\log A}$, set $E_{i'}$ contains all edges $e\in E^1$ that are incident to the vertices of $\bigcup_{y\in J_{i'}}(R(y)\cap V(G'))$. As before, $(E'_0,\ldots,E'_{\ceil{\log A}})$ is a partition of the set $E^1$ of edges. Therefore, there is an index $0\leq q'\leq \ceil{\log A}$ with $|E'_{q'}|\geq \frac{|E^1|}{2\log A}\geq \frac{|E^1|}{2\log n}\geq \frac{|E^0|}{4\log^2n}$. We then set $Y^*=J'_{q'}$. For each variable $y\in Y^*$, we let $R'(y)=R(y)\cap V(G')$, and for each variable $y\in \tilde Y\setminus Y^*$, we set $R'(y)=\emptyset$. We also let $E^2=E'_{q'}$. From the above discussion,  $|E^2|\geq \frac{|E^0|}{4\log^2 n}$, and, for every variable $y\in Y^*$, $2^{q'}\leq |R'(y)|<2^{y+1}$. Notice that every edge of $E^2$ is incident to a vertex of $\bigcup_{x\in X^*}R'(x)$ and a vertex of $\bigcup_{y\in Y^*}R'(y)$.
		
Our third and final step is to regularize the constraints. Recall that for each constraint $C=C(x,y)\in \tilde \cset$, we defined a set $E(C)$ of edges. Since $|R(x)|= A$ and $|R(y)|=A$, $|E(C)|\leq A^2\leq n$ must hold. We group all constraints $C\in \tilde \cset  $ into 
sets $\cset_0,\cset_1,\ldots,\cset_{\ceil{\log n}}$, where for all $0\leq j\leq \ceil{\log n}$, set $\cset_i$ contains all constraints $C\in \tilde \cset$ with $2^j\leq |E(C)\cap E^2|<2^{j+1}$. Note that, if $E(C)\cap E^2=\emptyset$, then constraint $C$ does not belong to any set. Next, we define a partition $E_0'',E_1'',\ldots,E_{\ceil{\log n}}''$ of the set $E^2$ of edges: for $0\leq j\leq \ceil{\log n}$, set $E''_j$ contains all edges in $\bigcup_{C\in \cset_j}(E(C)\cap E^2)$. It is easy to verify that $(E''_0,\ldots,E_{\ceil{\log n}}'')$ is indeed a partition of $E^2$. Therefore, there must be an index $0<r\leq \ceil{\log n}$, with $|E''_r|\geq \frac{|E^2|}{2\log n}\geq \frac{|E^0|}{8\log^3n}$. We let $\cset^*=\cset_r$ and $E^3=E''_r$.
Since every constraint $C\in \cset^*$ contributes at most $2^{r+1}$ edges to $E^3$, we get that:

\[|\cset^*|\geq \frac{|E^3|}{2^{r+1}} \geq \frac{|E^0|}{2^{r+4}\log^3n}\geq \frac{|\tilde \cset|}{2^{r+4}\cdot\gamma\cdot \alpha(n)\cdot \log^3n}. \]

 For every constraint $C\in \cset^*$, we let $E'(C)=E(C)\cap E^2$, and for every constraint $C\in \tilde \cset\setminus\cset^*$, we let $E'(C)=\emptyset$. We are now ready to define graph $G''$. Its vertex set is $\left (\bigcup_{x\in X^*}R'(X)\right )\cup \left (\bigcup_{y\in Y^*}R'(y)\right )$, and its edge set is $\bigcup_{C\in \cset^*}E'(C)=E^3$. 
It is immediate to verify, from the above discussion, that graph $G'$, sets $X^*,Y^*$ of variables, and set $\cset^*$ of constraints have all required properties.
\end{proof}
	
	
In the next observation, we establish some useful bounds on the cardinalities of the sets $X^*,Y^*$ of variables, and the set $\cset^*$ of constraints.
	
\begin{observation}\label{obs: bounds on sizes of sets}
All of the following bounds hold:

\begin{itemize}
	\item  $|X^*|\leq \frac{|\tilde  X|}{2^q}$; 
	\item 	$|Y^*|\leq \frac{|\tilde Y|}{2^{q'}}$;
	\item $|\cset^*|\leq 2d_1|X^*|\leq \frac{2d_1|\tilde X|}{2^q}$; and
	\item $|\cset^*|\leq 2d_2|Y^*|\leq \frac{2d_2|\tilde Y|}{2^{q'}}$.
\end{itemize}
\end{observation}
	
\begin{proof}
	From the definition of the instance $(G,k_1,k_2)$ of \DS, graph $G'$ contained at most $k_1=|\tilde X|$ vertices of $\bigcup_{x\in \tilde X}R(x)$, and at most $k_2=|\tilde Y|$ vertices of $\bigcup_{y\in \tilde Y}R(y)$. Since, for every variable $x\in X^*$, $R'(x)\subseteq V(G')$ and $|R'(x)|\geq 2^q$, we get that $|X^*|\leq \frac{|\tilde X|}{2^q}$. Similarly, $|Y^*|\leq \frac{|\tilde Y|}{2^{q'}}$. 
	
	Recall that, since $\tilde H$ is a nice subgraph of $H$, for every vertex $x\in \tilde H$, $\deg_{\tilde H}(x)\leq \deg_H(x)\leq 2d_1$, and so $x$ may participate in at most $2d_1$ constraints of $\tilde \cset$. Since $\cset^*\subseteq \tilde \cset$ and $X^*\subseteq \tilde X$, every variable $x\in X^*$ may participate in at most $2d_1$ constraints of $\cset^*$. Therefore, $|\cset^*|\leq 2d_1|X^*|$. 
	
	Similarly, since $\tilde H$ is a nice subgraph of $H$, for every vertex $y\in \tilde Y$, $\deg_{\tilde H}(y)\leq 2d_2$. Using the same arguments as before, $|\cset^*|\leq 2d_2|Y^*|$.
	\end{proof}
	
	
Recall that, from \Cref{claim: regularization}, $|\cset^*|\geq \frac{|\tilde \cset|}{2^{r+4}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$. Since graph $\tilde H$ is a nice subgraph of $H$, we get that, for every vertex $y\in \tilde Y$, $\deg_{\tilde H}(y)\geq d_2$. Therefore, $|\tilde \cset|\geq |\tilde Y|\cdot d_2$, and so:

\begin{equation}
|\cset^*|\geq \frac{d_2\cdot |\tilde Y|}{2^{r+4}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}.  \label{eq2}
\end{equation} 	


		
Similarly, from the definition of a nice subgraph, $|\tilde \cset|\geq \frac{d_1}{4\log n}\cdot |\tilde X|$, and so:

\begin{equation}
|\cset^*|\geq \frac{d_1\cdot |\tilde X|}{2^{r+6}\cdot \gamma\cdot \alpha(n)\cdot \log^4n}.  \label{eq3}
\end{equation} 	
	
	
	Lastly, we show that both $2^q,2^{q'}$ are close to $2^r$, in the following corollary of \Cref{obs: bounds on sizes of sets}.
	
	\begin{corollary}\label{cor: q q' and r}
		The following inequalities hold:
		
		\begin{itemize}
			\item 	$\frac{2^r}{2d(n)}\leq 2^{q}\leq 2^{r+7}\cdot \gamma\cdot \alpha(n)\cdot \log^4n$; and
			\item $\frac{2^r}{2d(n)}\leq 2^{q'}\leq 2^{r+5}\cdot \gamma\cdot \alpha(n)\cdot \log^3n$.
		\end{itemize}
	\end{corollary}
	
	\begin{proof}
		Consider some constraint $C=C(x,y)\in \cset^*$, and recall that $|E'(C)|\geq 2^r$. From the definition of the $d$-to-$d$ instances, every vertex $v(x,a)\in R(x)$ may be incident to at most $d(n)$ edges of $E(C)$. Since all edges of $E'(C)$ are incident to vertices of $R'(x)$, and $|R'(x)|\leq 2^{q+1}$, we get that $|E'(C)|\leq d(n)\cdot |R'(x)|\leq d(n)\cdot 2^{q+1}$. We conclude that $2^r\leq d(n)\cdot 2^{q+1}$.
		
		Similarly, every vertex $v(y,A)\in R(y)$ may be incident to at most $d(n)$ edges of $E(C)$. Since all edges of $E'(C)$ are incident to vertices of $R'(y)$, and $|R'(y)|\leq 2^{q'+1}$, we get that $|E'(C)|\leq d(n)\cdot 2^{q'+1}$.
		This proves the inequalities $\frac{2^r}{2d(n)}\leq 2^{q}$ and $\frac{2^r}{2d(n)}\leq 2^{q'}$.  
		
		
		Next, we prove that 	$2^{q'}\leq 2^{r+6}\cdot \gamma\cdot \alpha(n)\cdot \log^3n$. %Recall that, from \Cref{obs: bounds on sizes of sets}, $|\cset^*|\geq \frac{|\tilde \cset|}{2^{r+5}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$. Since graph $\tilde H$ is a nice subgraph of $H$, we get that, for every vertex $y\in \tilde Y$, $\deg_{\tilde H}(y)\geq d_2$. Therefore, $|\tilde \cset|\geq |\tilde Y|\cdot d_2$, and so:
	Recall that, from Inequality \ref{eq2}, $|\cset^*|\geq	\frac{d_2\cdot |\tilde Y|}{2^{r+5}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$.
		On the other hand, from the definion of a nice subgraph, every variable $y\in Y^*$ may participate in at most $2d_2$ constraints of $\cset^*$, and, from \Cref{obs: bounds on sizes of sets}, 	$|Y^*|\leq \frac{|\tilde Y|}{2^{q'}}$. Therefore: 
		
		
		\begin{equation}
		|\cset^*|\leq 2d_2\cdot |Y^*|\leq  \frac{2d_2|\tilde Y|}{2^{q'}}.
		\end{equation}
		
		Combining the two inequalities, we get that:	$2^{q'}\leq 2^{r+5}\cdot \gamma\cdot \alpha(n)\cdot \log^3n$.
		
		
		
		
		
		Lastly, we prove that 	$2^q\leq 2^{r+7}\cdot \gamma\cdot \alpha(n)\cdot \log^4n$. 
Recall that, from Inequality \ref{eq3}, 
$|\cset^*|\geq \frac{d_1\cdot |\tilde X|}{2^{r+6}\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$ holds.


As before, from the definion of a nice subgraph, every variable $x\in X^*$ may participate in at most $2d_1$ constraints of $\cset^*$, and, from \Cref{obs: bounds on sizes of sets}, 	$|X^*|\leq \frac{|\tilde X|}{2^{q}}$. Therefore: 


\begin{equation}
|\cset^*|\leq 2d_1\cdot |X^*|\leq  \frac{2d_1\cdot |\tilde X|}{2^{q}}.
\end{equation}

Combining the two inequalities together, we get that:	$2^{q}\leq 2^{r+7}\cdot \gamma\cdot \alpha(n)\cdot \log^4n$.		
\end{proof}
	
	
\subsubsection{Step 4: Certifying that $H$ is a Good Graph or Computing a Subgraph of $H$}

%Let $z=\sqrt{\frac{\beta}{2^{23}\cdot \gamma^3\cdot (\alpha(n))^3\cdot \log^{13}n}}$. 
We consider two cases, depending on whether $2^r\leq \beta$ holds. We start by showing that, if $2^r\leq \beta$, then graph $H$ is $\beta^3$-good.

\begin{observation}\label{obs: good graph}
	If $2^r\leq \beta$, then graph $H$ is $\beta^3$-good.
\end{observation}
\begin{proof}
We show that there exists an assignment to variables of $X\cup Y$ that satisfies at least $|\cset|/\beta^3$ constraints of $\cset$. In order to do it, we show a randomized algorithm that computes assignments to variables of $X\cup Y$, such that the expected number of satisfied constraints is at least $|\cset|/\beta^3$.

The assignments are computed as follows. Consider a variable $x\in X$. If $x\not\in X^*$, then we assign to $x$ an abitrary value from $[A]$. Assume now that $x\in X^*$. Recall that we have defined a set $R'(x)\subseteq R(x)$ of vertices, whose cardinality is at most $2^{q+1}$. Set $R'(x)$ of vertices naturally defines a collection $\hat A(x)=\set{a\in [A]\mid v(x,a)\in R'(x)}$ of assignments to variable $x$, with $|\hat A(x)|\leq 2^{q+1}$. We choose an assignment $a\in \hat A(x)$ uniformly at random, and assign value $a$ to $x$.

Assignments to variables of $Y$ are defined similarly. Consider a variable $y\in Y$. If $y\not\in Y^*$, then we assign to $y$ an abitrary value from $[A]$. Assume now that $y\in Y^*$. Recall that we have defined a set $R'(y)\subseteq R(y)$ of vertices, whose cardinality is at most $2^{q'+1}$. Set $R'(y)$ of vertices naturally defines a collection $\hat A(y)=\set{a\in [A]\mid v(y,a)\in R'(y)}$ of assignments to variable $y$, with $|\hat A(y)|\leq 2^{q'+1}$. We choose an assignment $a'\in \hat A(y)$ uniformly at random, and assign value $a'$ to $y$.

Recall that we have computed, in \Cref{claim: regularization}, a collection $\cset^*\subseteq \cset$ of constraints, with $|\cset^*|\geq \frac{|\tilde \cset|}{2^{r+4}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$. Consider now any constraint $C=C(x,y)\in \cset^*$, and recall that $x\in X^*,y\in Y^*$ must hold. Recall that graph $G''$ contains a collection $E'(C)\subseteq E(C)$ of edges, with $|E'(C)|\geq 2^r$. Consider now any such edge $e=(v(x,a),v(y,A))$. We say that edge $e$ wins if $x$ is assigned value $a$, and $y$ is assigned value $a'$. The probability that edge $e$ wins is at least $\frac{1}{2^{q+1}\cdot 2^{q'+1}}$. Notice that at most one edge of $E'(C)$ may win, and so the probability that any edge of $E'(C)$ wins is at least $\frac{|E'(C)|}{2^{q+1}\cdot 2^{q'+1}}\geq \frac{2^r}{2^{q+1}\cdot 2^{q'+1}}$. If any edge of $E'(C)$ wins, the constraint $C$ is satisfied by the assignment that the algorithm chooses. Therefore, the probability that a constraint $C\in \cset^*$ is satisfied is at least $ \frac{2^r}{2^{q+1}\cdot 2^{q'+1}}$.

Overall, the expected number of constraints that are satisfied by the assignemnt is at least:

\[\frac{|\cset^*|\cdot 2^r}{2^{q+1}\cdot 2^{q'+1}}\geq \frac{|\tilde \cset|}{2^{6}\cdot \gamma\cdot \alpha(n)\cdot 2^q\cdot 2^{q'}\cdot \log^3n}\]

Recall that, from \Cref{claim: regularizing constraint graph}, $|\tilde \cset|=|E(\tilde H)|\geq \frac{|E(H)|}{8\log^2n}=\frac{|\cset|}{8\log^2n}$, and, from \Cref{cor: q q' and r}, $2^q\cdot 2^{q'}\leq 2^{2r+12} \cdot \gamma^2\cdot (\alpha(n))^2\cdot \log^7n\leq 2^{12}\cdot \beta^2\cdot \gamma^2\cdot (\alpha(n))^2\cdot \log^7n$, since we have assumed that $2^r\leq \beta$.
Therefore, the expeced number of constraints of $\cset$ that are satisfied by the assignment is at least:

\[\frac{|\tilde \cset|}{2^{6}\cdot \gamma\cdot \alpha(n)\cdot 2^q\cdot 2^{q'}\cdot \log^3n}\geq \frac{|\cset|}{2^{9}\cdot \gamma\cdot \alpha(n)\cdot 2^q\cdot 2^{q'}\cdot \log^5n}\geq  \frac{|\cset|}{2^{21}\cdot \beta^2\cdot \gamma^3\cdot (\alpha(n))^3 \cdot \log^{12}n}\geq \frac{|\cset|}{\beta^3},\]


since $\beta \geq 2^{23}\gamma^3(\alpha(n))^3\log^{12}n$.
%since $z=\sqrt{\frac{\beta}{2^{23}\cdot \gamma^3\cdot (\alpha(n))^3\cdot \log^{13}n}}$.

We conclude that there is an assignment to the variables of $X\cup Y$ that satisfies at least $|\cset|/\beta$ constraints of $\cset$, and so graph $H$ is $\beta$-good.
\end{proof}

If $2^r\leq \beta$, then we terminate the algorithm and report that graph $H$ is $\beta$-good. 

From now on we assume that $2^r>\beta$. In this case, we return a subgraph  a subgraph $H'=(X',Y',E')$ of $H(\iset)$, that is defined as follows: $X'=X^*$, $Y'=Y^*$, and $E'=E^*$. We now verify that this graph has all required properties.

Recall that, from \Cref{obs: bounds on sizes of sets}, $|X^*|\leq  \frac{|\tilde  X|}{2^q}\leq \frac{|X|}{2^q}$, from \Cref{cor: q q' and r}, $2^q\geq \frac{2^r}{2d(n)}$, and, from our assumption, $2^r>\beta$. Therefore:

\[|X^*|\leq  \frac{|X|}{2^q}\leq \frac{|X|\cdot 2d(n)}{2^r}\leq \frac{2d(n)}{\beta}\cdot |X|. \]

Similarly, from \Cref{obs: bounds on sizes of sets}, $|Y^*|\leq  \frac{|\tilde  Y|}{2^{q'}}\leq \frac{|Y|}{2^{q'}}$, from \Cref{cor: q q' and r}, $2^{q'}\geq \frac{2^r}{2d(n)}$, and, from our assumption, $2^r>\beta$. Therefore:

\[|Y^*|\leq  \frac{|Y|}{2^{q'}}\leq \frac{|Y|\cdot 2d(n)}{2^r}\leq \frac{2d(n)}{\beta}\cdot |Y|. \]

It now only remains to show that:  $|E'|\geq \frac{\vol_H(X^*\cup Y^*)}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^5n}$.


Recall that, from Inequality \ref{eq3}, 
$|\cset^*|\geq \frac{d_1\cdot |\tilde X|}{2^{r+6}\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$ holds. Since, from \Cref{cor: q q' and r}, $2^r\leq 2^q\cdot 2d(n)$, we get that $|E'|=|\cset^*|\geq \frac{d_1\cdot |\tilde X|}{2^{q+7}\cdot d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$. At the same time, from the definition of a nice graph, for every vertex $x\in X^*$, $\deg_H(x)\leq 2d_1$, so $\vol_H(X^*)\leq 2d_1\cdot |X^*|\leq \frac{2d_1\cdot |\tilde X|}{2^q}$, since $|X^*|\leq \frac{|\tilde  X|}{2^q}$ from \Cref{obs: bounds on sizes of sets}. Therefore, 
$|E'|\geq \frac{\vol_H(X^*)}{64d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}
$.

Similarly, from Inequality \ref{eq2}, $|\cset^*|\geq	\frac{d_2\cdot |\tilde Y|}{2^{r+4}\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$.
Since, from \Cref{cor: q q' and r}, $2^r\leq 2^{q'}\cdot 2d(n)$, we get that $|E'|=|\cset^*|\geq \frac{d_2\cdot |\tilde Y|}{2^{q'+5}\cdot d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^3n}$. At the same time, from the definition of a nice graph, for every vertex $y\in Y^*$, $\deg_H(y)\leq 2d_2$, so $\vol_H(Y^*)\leq 2d_2\cdot |Y^*|\leq \frac{2d_2\cdot |\tilde Y|}{2^{q'}}$, since $|Y^*|\leq \frac{|\tilde  Y|}{2^{q'}}$ from \Cref{obs: bounds on sizes of sets}. Therefore, 
$|E'|\geq \frac{\vol_H(Y^*)}{64d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^3n}
$.

Altogether, we get that $|E'|\geq \frac{\vol_H(X^*\cup Y^*)}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$.



 



%	\paragraph{Case 1: $2^r\leq \beta$.} In this case, we compute an assignment to the variables of $\hat X\cup \hat Y$ that satisfies a large fraction of the constraints in $E'$. In order to compute the assignment, every variable $x\in X^*$ chooses one of its at most $2^{q+1}$ assignments in $S'(x)$ uniformly at random, and similarly, every variable $y\in Y^*$ chooses one of its assignments in $S'(y)$ uniformly at random. We now show that this assignment satisfies many constraints. In order to do so, we show that (i) $|E^*|$ is quite large; and (ii) every constraint in $E^*$ is satisfied with a high enough probability. In order to show (i), recall that:
	
%	\[|E^*|\cdot 2^r\geq \frac{|\hat E|}{2\alpha\log^3A} \geq \frac{|E(H')|}{8\alpha\log^3A\log^2N}. \]
	
%	Therefore:
	
%	\[|E^*|\geq \frac{|E(H')|}{8\cdot 2^r\alpha\log^3A\log^2N}\geq\frac{|E(H')|}{8\cdot \beta\alpha\log^3A\log^2N}\geq\frac{|E(H')|}{\beta^2}.\]
	
%	On the other hand, the probability that a constraint $C\in E^*$ is satisfied is at least:
	
%	\[\frac{2^r}{2^{q+1}\cdot 2^{q'+1}}\geq \frac{2^r}{2^{4r+6}\alpha^2 \log N\log^6A}\geq \frac{1}{2^{3r+6}\alpha^2\log N\log^6A}\geq \frac{1}{\beta^4}.\]
	
%	Therefore, the expected number of constraints we satisfy is at least $\frac{|E(H')|}{\beta^6}$.
	

	
	






\newpage

==> DkS-outer-thm-backup.tex <==
\begin{theorem}\label{thm: partition or solution for no instance}
	Assume that there exists an efficient $\alpha(N)$-approximation algorithm $\aset$ for the \DS problem, where $N$ is the number of vertices in the input graph. Then there is an efficient algorithm, that, given an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP and parameters $n,\gamma,\beta\geq 1$, so that $\size(\iset)\leq n$,  $\beta \geq 2^{23}\gamma^3(\alpha(n))^3(\log n)^{12}$, and $\iset$ is a $d(n)$-to-$d(n)$ instance of \BCSP, does one of the following:
	
	\begin{itemize}
		\item either correctly establishes that graph $H(\iset)$ is $\beta^3$-good; or
		
		\item computes a $\gamma$-bad set $\cset'\subseteq \cset$ of constraints, with $|\cset'|\geq \frac{|\cset|}{8\log^2n}$; or
		\item  computes a subgraph $H'=(X',Y',E')$ of $H(\iset)$, for which the following hold:
		\begin{itemize}
			\item $|X'|\leq \frac{2d(n)\cdot |X|}{\beta}$;
			\item $|Y'|\leq \frac{2d(n)\cdot |Y|}{\beta}$; and
			\item $|E'|\geq \frac{\vol_H(X'\cup Y')}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$.
		\end{itemize}
	\end{itemize} 
\end{theorem}


We prove \Cref{thm: partition or solution for no instance} in Section \Cref{subsec: proof of inner thm for DkS}, after we complete the proof of ? using it.

We start with the following corollary of \Cref{thm: partition or solution for no instance}.








\begin{corollary}\label{thm: general partition of solution}
	Assume that there exists an efficient $\alpha(N)$-approximation algorithm $\aset$ for the \DS problem, where $N$ is the number of vertices in the input graph. Then there is an efficient algorithm, whose input consists of an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP and parameters $n,\gamma,\beta\geq 1$, so that $\size(\iset)\leq n$,  $\beta \geq 2^{23}\gamma^3(\alpha(n))^3(\log n)^{12}$, and $\iset$ is a $d(n)$-to-$d(n)$ instance of \BCSP. The algorithm  returns a partition $(E_1,E_2)$ of $E(H(\iset))$, where $E_1$ is a $\gamma$-bad set of edges, and:

\begin{itemize}
	\item either the algorithm correctly certifies that $E_2$ is a $\beta^3$-good set of edges; or

\item it computes a subgraph $H'=(X',Y',E')$ of $H(\iset)$, with $E(H')\subseteq E_2$, for which the following hold:
	\begin{itemize}
		\item $|X'|\leq \frac{2d(n)\cdot |X|}{\beta}$;
		\item $|Y'|\leq \frac{2d(n)\cdot |Y|}{\beta}$; and
		\item $|E'|\geq \frac{|E^*_2|}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$, where $E^*_2$ is a set of edges containing every edge $e\in E_2$ with exactly one endpoint in $V(H')$.
	\end{itemize}
\end{itemize} 
\end{corollary}	


\begin{proof}
The algorithm is iterative. We start with $E_1=\emptyset$, $E_2=E(H(\iset))$ and $H=H(\iset)$. We then iterate. In every iteration, we compute a graph $H'=H\setminus E_1$. We denote by $\cset'=\Phi(E(H'))$ the set of all constraints of $\cset$ corresponding to the edges of $H'$.  Notice that graph $H'$ naturally defines a $d(n)$-to-$d(n)$ instance $\iset'$ of \BCSP, whose size is at most $n$, that corresponds to the subset $\cset'\subseteq \cset$ of constraints. 
We apply the algorithm from \Cref{thm: partition or solution for no instance} to instance $\iset'$. If the outcome of the algorithm is a  $\gamma$-bad set $\cset''\subseteq \cset'$ of constraints, then we let $\tilde E=\set{e_C\mid C\in \cset''}$ be the set of edges of $H'$ corresponding to the constraints of $\cset''$. We add the edges of $\tilde E$ to $E_1$, remove them from $E_2$, and continue to the next iteration.

If the algorithm of the algorithm from \Cref{thm: partition or solution for no instance} certifies that graph $H'$ is $\beta^3$-good, then we terminate the algorithm with the current partition $(E_1,E_2)$ of $E(H)$, and certify that the set $E_2$ of edges is $\beta^3$-good.

Otherwise, the outcome of of the algorithm from \Cref{thm: partition or solution for no instance} must be a subgraph $H''=(X',Y',E')$ of $H'$, with $|X'|\leq \frac{2d(n)\cdot |X|}{\beta}$ and $|Y'|\leq \frac{2d(n)\cdot |Y|}{\beta}$. The algorithm also guarantees that $|E'|\geq \frac{\vol_{H'}(X'\cup Y')}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$.

Let $E^*_2$ be the set of edges containing every edge $e\in E_2$ with exactly one endpoint in $V(H'')$. Since $E(H')=E_2$, it is immediate to verify that $|E^*_2|\leq \vol_{H'}(X'\cup Y')$. Therefore, we are guaranteed that $|E'|\geq \frac{\vol_{H'}(X'\cup Y')}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$. We return the current partition $(E_1,E_2)$ of $E(H)$ and subgraph $H''$ of $H(\iset)$, and terminate the algorithm.
\end{proof}




We then obtain the following corollary.
\begin{corollary}\label{cor: a phase outer DkS}
	Assume that there exists an efficient $\alpha(N)$-approximation algorithm $\aset$ for the \DS problem, where $N$ is the number of vertices in the input graph. Then there is an efficient algorithm, whose input consists of an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP and parameters $n,\gamma,\beta\geq 1$, so that $\size(\iset)\leq n$,  $\beta \geq 2^{23}\gamma^3(\alpha(n))^3(\log n)^{12}$, and $\iset$ is a $d(n)$-to-$d(n)$ instance of \BCSP. The algorithm  returns a partition $(E_1,E_2,E_3)$ of $E(H(\iset))$, where $E_1$ is a $\gamma$-bad set of constraints, $E_2$ is a $\beta^3$-good set of constraints, and $|E_1\cup E_2|\geq \frac{|E(H(\iset))|}{\beta}$.
\end{corollary}

\begin{proof}
For convenience, we denote $H=H(\iset)$. Our algorithm uses a parameter $\eta=256 8d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n$.

The algorithm is iterative. Over the course of the algorithm, we maintain a collection $\hset$ of subgraphs of $H$, and another subgraph $H^g$ of $H$. We will ensure that, throughout the algorithm, all graphs in $\hset\cup \set{H^g}$ are mutually disjoint in their vertices. We denote by $E^g=E(H^g)$ and $E^1=\bigcup_{H'\in \hset}E(H')$. Additionally, we maintain another set $E^b$ of edges of $H$, that is disjoint from $E^g\cup E^1$, and we denote by $E^0=E(H)\setminus (E^g\cup E^b\cup E^1)$ the set of all remaining edges of $H$.
We ensure that the following invariants hold throughout the algorithm.




\begin{properties}{I}
	\item set $E^g=E(H^g)$ of edges is $\beta$-good; \label{inv: good edges};
	\item set $E^b$ of edges is $\gamma$-bad;\label{inv: bad edges} and
	
	\item all graphs in $\hset\cup \set{H^g}$ are disjoint in their vertices. \label{inv: disjoint graphs}
	
%	\item If we denote by $H_1$ and $H_2$ the sub-graphs of $\tilde H$ induced by the edges of $E_1$ and $E_2$, respectively, then all graphs in $\hset$ are vertex-disjoint from both $H_1$ and $H_2$ (but we allow $H_1$ and $H_2$ to share vertices).
\end{properties}

Intuitively, we will start with the set $\hset$ containing a single graph $H$, and $E^g=E^b=E^0=\emptyset$. As the algorithm progresses, we will iteratively add edges to sets $E^g,E^b$ and $E^0$, while partitioning the graphs in $\hset$ into smaller subgraphs. The algorithm will terminate once $\hset=\emptyset$. The key in the analysis of the algorithm is to ensure that $|E^0|$ is relatively small when the algorithm terminates. We do so via a charging scheme: we assign a budget to every edge of $E^1\cup E^g\cup E^b$, that evolves over the course of the algorithm, and we keep track of this budget over the course of the algorithm.

In order to define vertex budgets, we will assign, to every graph $H\in \hset$ a \emph{level}, that is an integer between $1$ and $\ceil{\log n}$. We will ensure that, throughout the algorithm, the following additional invariants hold:

\begin{properties}[3]{I}
\item If $H'\in \hset$ is a level-$i$ graph, then the budget of every edge $e\in E(H')$ is at most $\eta^i$; and \label{prop: charge each edge}

\item at every point of the algorithm's excution, the total budget of all edges in $E^g\cup E^b\cup E^1$ is at least $|E(H)|$.\label{prop: total budget}
\end{properties}

Intuitively, at the end of the algorithm, we will argue that the level of every graph in $\hset$ is not too large, and that the budget of every edge in $E^g\cup E^b\cup E^1$ is not too small. Since the total budget of all edges in  $E^g\cup E^b\cup E^1$ is at least $|E(H)|$, it will then follow that $|E^g\cup E^b\cup E^1$ is sufficiently large.
We now proceed to describe the algorithm.

$E_0$ - deleted. 
$E_1$ - good 
$E_2$: bad

$E_3$: in graphs of $\hset$.


\paragraph{Initialization.}
At the beginning of the algorithm, we set $E^0=E^g=E^b=\emptyset$, and we  let $\hset$ contain a single graph $H$, which is assigned level $0$. Note that $E^1=E(H)$ must hold. Every edge $e\in E(H)$ is assigned budget $b(e)=1$. Clearly, the total budget of all edges of $E^1\cup E^g\cup E^b$ is $B=\sum_{e\in E^1\cup E^g\cup E^b}b(e)=|E(H)|$.

The algorithm performs iterations, as long as $\hset\neq \emptyset$. In every iteration, we select an arbitrary graph $H'\in \hset$ to process. We now describe a single iteration.



\paragraph{Iteration description.}
We now describe an iteration where some graph $H'\in \hset$ is processed. We assume that graph $H'$ is assigned level $i$. Notice that graph $H'$ naturally defines an instance $\iset'=(X',Y',A,\cset',\set{G_C}_{C\in \cset'})$ of \BCSP, where $X'=V(H')\cap X$, $Y'=V(H')\cap Y$, $\cset'=\set{C\in \cset\mid e_C\in E(H')}$, and the graphs $G_C$ for constraints $C\in \cset'$ remain the same as in instance $\iset$. Clearly, $\size(\iset')\leq \size(\iset)\leq n$, and $H(\iset')=H'$. Furthermore, instance $\iset'$ remains a $d(n)$-to-$d(n)$ instance. We apply the algorithm from \Cref{thm: general partition of solution} to instance $\iset'$, with parameters $n,\gamma,\beta$ remaining unchanged. Consider the partition $(E_1,E_2)$ of $E(H')$ that the algorithm returns. Recall that the set $E_1$ of edges is $\gamma$-bad. We add the edges of $E_1$ to set $E^b$. From Invariant \ref{inv: bad edges} and \Cref{obs: bad constraints}, set $E^b$ of edges continues to be $\gamma$-good. If the algorithm from \Cref{thm: general partition of solution} certified that $E_2$ is a $\beta^3$-good set of edges, then we update graph $H^g$ to be $H^g\cup H'\setminus E_1$, and we add the edges of $E_1$ to set $E^g$. We then remove graph $H'$ from $\hset$, and continue to the next iteration. Note that, from \Cref{obs: good constraints} and Invariants \ref{inv: good edges} and \ref{inv: disjoint graphs}, the set $E^g$ of edges continues to be $\beta^3$-good. It is easy to verify that all remaining invariants also continue to hold.

From now on we assume that the algorithm from \Cref{thm: general partition of solution} returned a subgraph $H''=(X'',Y'',E'')$ of $H'$, with $E''\subseteq E_2$, such that $|X''|\leq \frac{2d(n)\cdot |X'|}{\beta}$ and $|Y''|\leq \frac{2d(n)\cdot |Y'|}{\beta}$. In particular, $|V(H'')|=|X''|+|Y''|\leq \frac{2d(n)}{\beta}\cdot (|X'|+|Y'|)\leq  \frac{2d(n)}{\beta}\cdot |V(H')|$.
Additinally, if we denote by $E^*_2$ the subset of edges of $E_2$ containing all edges with exactly one endpoint in $X''\cup Y''$, then
$|E''|\geq \frac{|E^*_2|}{128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n}$ must hold.
We let $H^*$ be the graph obtained from $H'\setminus E_1$, by deleting the vertices of $H''$ from it, so $V(H^*)\cup V(H'')=V(H')$, and $E(H^*)\cup E(H'')\cup E^*_2=E_2$. We remove graph $H'$ from $\hset$, and we add graphs $H''$ and $H^*$ to $\hset$, with graph $H''$ assigned level $(i+1)$, and graph $H^*$ assigned level $i$. We also add the edges of $E_2^*$ to $E^0$, and we update the set $E^1$ of edges to contain all edges of $\bigcup_{\tilde H\in \hset}E(\tilde H)$. Since we did not modify graph $H^g$ in the current iteration, it is immediate to verify that Invariants \ref{inv: good edges}--\ref{inv: disjoint graphs} continue to hold. Next, we update the budgets of edges, to ensure that 
Invariants \ref{prop: charge each edge} and \ref{prop: total budget} continue to hold. Intuitively, the edges of $E^*_2$ are now added to set $E^0$, so we need to distribute their budget among the edges of $E(H'')$, to ensure that the total budget of all edges in $E^g\cup E^b\cup E^1$ does not decrease. This will ensure that Invariant \ref{prop: total budget} continues to hold. At the same time, since the level of graph $H''$ is $(i+1)$, while the level of graph $H'$ was $i$, we can increase the budgets of the edges of $E(H')$ and still maintain Invariant \ref{prop: charge each edge}.

Formally, recall that \Cref{thm: general partition of solution} guarantees that $|E^*_2|\leq |E''|\cdot (128d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n)=\frac{|E''|\cdot \eta} 2$. From Invariant \ref{prop: charge each edge}, the current budget of every edge in $E''\cup E^*_2$ is bounded by $\eta^i$. Therefore, at the beginning of the current iteration:

\[\sum_{e\in E''\cup E^*_2}b(e)\leq \eta^i\cdot \left(|E^*_2|+|E''|\right )\leq \eta^i\cdot |E''|\cdot \left(1+\frac{\eta}{2}\right )<\eta^{i+1}\cdot |E''|.
\]

We set the budget of every edge in $E''$ to be $\eta^{i+1}$, and leave the budgets of all other edges unchanged. It is easy to verify that $\bigcup_{e\in E^g\cup E^b\cup E^1}b(e)$ does not decrease in the current iteration, so Invariant \ref{prop: total budget} continues to hold. It is also easy to verify that Invariant \ref{prop: charge each edge} continues to hold. Therefore, all invariants continue to hold at the end of the iteration. This completes the description of an iteration.


%Consider now some graph $H'\in \hset$, and assume that it belongs to level $i$. In order to process $H'$, we apply Theorem~\ref{thm: general partition of solution} to it. Assume that we obtain a partition $(E_1',E_2')$ of $E(H')$. We consider two cases. First, if $E_2'$ is a good set of constraints, then we add the edges of $E_1'$ to $E_1$, the edges of $E_2'$ to $E_2$, and delete $H'$ from $\hset$. 

%Assume now that the algorithm from Theorem~\ref{thm: general partition of solution} returns a subgraph $H''$ of $H'\setminus E'_1$. Let $V_1=V(H'')$ and $V_2=V(H')\setminus V_1$. Let $\tilde E=E(H'')$ and let $\tilde E'=E_{H'}(V_1,V_2)\setminus E_1'$. Finally, let $\tilde E''=E_{H'}(V_2)\setminus E_1'$. Notice that $\tilde E,\tilde E',\tilde E''$ and $E'_1$ partition the edges of $E(H')$. We add the edges of $E'_1$ to $E_1$ (recall that $E'_1$ is a bad set of constraints, and from Observation~\ref{obs: good and bad constraints under union}, so is $E'_1\cup E_1$. We also add the edges of $\tilde E'$ to $E_0$. We remove $H'$ from $\hset$, and add two new graphs to $\hset$ instead: 
%graph $H''$, that belongs to level $(i+1)$, and graph $H'''$ that belongs to level $i$, whose vertex set is $V_2$, and edge set is $\tilde E''$.
%Next, we update the charges of all edges. The charge of every edge in $E(H''')$ remains unchaged. We increase the charge to every edge in $E(H'')$, so that they can cover the charge of every edge in $\tilde E'$. Recall that, since $H'$ is a level-$i$ graph, the charge to every vertex of $H'$ is at most $(2\eta)^i$. Recall also that Theorem~\ref{thm: general partition of solution} guarantees that 
%$|E(H'')|\geq |\tilde E'|/\eta$. Since every edge in $E(H'')\cup \tilde E'$ has a charge of at most $(2\eta)^i$, we can distribute the charges of the edges in $\tilde E'$ among the edges of $E(H'')$, so that every edge in $E(H'')$ gets an additional charge of at most $\eta\cdot (2\eta)^i$, and so the new charge of every edge in $E(H'')$ is at most $(2\eta)^{i+1}$, as required. We set the charge of every edge in $\tilde E'$ to $0$.



%Throughout the algorithm, we maintain a bad subset $E_1\subseteq E(\tilde H)$ of constraints, a good subset $E_2\subseteq E(\tilde H)$ of constraints, a subset $E_0\subseteq E(\tilde H)$ of \emph{deleted constraints}, and a collection $\hset$ of vertex-disjoint subgraphs of $\tilde H$. Let $E_3=\bigcup_{H'\in \hset}E(H')$. We also assign, to every graph $H'\in \hset$ a \emph{level}. Each edge $e$ of $E_1\cup E_2\cup E_3$ is assigned a \emph{charge} (which changes throughout the algorithm). We ensure that the total charge of all edges in $E_1\cup E_2\cup E_3$ is at least $|E(\tilde H)$. We also ensure that the following invariantes hold.


%Additionally, for accounting purposes, we assign to every graph of $\tilde H$ a \emph{level}, which is a non-negative integer.
%When the algorithm starts, we set $E_1=E_2=E_0=\emptyset$, and $\hset$ contains a single graph $\tilde H$, which is a level-$0$ graph. Every edge $e\in E(\tilde H)$ is assigned a charge of $1$. The algorithm continues as long as $\hset\neq \emptyset$. In every iteration, we select an arbitrary graph $H'\in \tilde H$ and process it.



The algorithm terminates when $\hset=\emptyset$. Clearly, we obtain a partition $(E^g,E^b,E^0)$ of $E(H)$ into disjoint subsets, where the set $E^b$ of edges is $\gamma$-bad, and the set $E^g$ of edges is $\beta^3$-good. It remains to show that $|E^g\cup E^b|\geq \frac{|E(H)|}{\beta}$.
We use the edge budgets in order to prove this. We start with the following key observation.

\begin{observation}\label{obs: graph level}
	Throughout the algorithm, if $H\in \hset$ is any cluster, and the level assigned to $H$ is $L$, then $L\leq \frac{\log n}{\log\left(\frac{\beta}{2d(n)}\right )}$.
\end{observation}
\begin{proof}
	Consider any graph $H''$ that was added to set $\hset$ at any time during the algorithm's execution, and assume that $H''$ was assigned level $i$. Consider the iteration during which $H''$ was added to $\hset$, and let $H'\in \hset$ be the graph that was processed during that iteration. We refer to graph $H'$ as the \emph{parent-graph} of $H''$. Note that the level of $H'$ is either $i$ or $(i-1)$. Assume that it is the latter. Then, from the algorithm's description, $|V(H'')|\leq  \frac{2d(n)}{\beta}\cdot |V(H')|$ must hold.
	
	We can now construct a \emph{partitioning tree}, that contains a vertex $v(H')$ for every graph $H'$ that was ever present in $\hset$ over the course of the algorithm, an an edge between vertices $v(H')$ and $v(H'')$ whenever graph $H'$ is a parent-graph of graph $H''$. The root of the tree is $v(H)$. Consider now again some graph $H''$, and the unique path $P$ in the partitioning tree, connecting $v(H)$ to $v(H'')$. Denote the vertices on this path by $v(H)=v(H_0),v(H_1),\ldots,v(H_r)=v(H'')$, and assume that these vertices appear on path $P$ in this order. For all $1\leq i\leq r$, denote the level of graph $H_i$ by $L_i$. Then $0=L_1\leq L_2\leq\cdots\leq L_r$ must hold. Moreover, if, for every index $0<i\leq r$, either $L_i=L_{i-1}$; or $L_i=L_{i-1}+1$. In the latter case, $|V(H_i)|\leq |V(H_{i-1})|\cdot \frac{2d(n)}{\beta}$. Denote $L^*= \frac{\log n}{\log\left(\frac{\beta}{2d(n)}\right )}$, and Assume for contradiction that $L_r>L^*$. Then there is a collection $J\subseteq \set{1,\ldots,r}$ of at least $L^*+1$ indices $i$, for which $L_i=L_{i-1}+1$. But then:
	
	\[|V(H'')|\leq n\cdot\left(\frac{2d(n)}{\beta}\right )^{L^*+1}<1, \]
	
	a contradiction.
	\end{proof}

%We start by showing that the largest level of any cluster in $\hset$ is bounded by $\log N/\log (\beta/2d)$. Indeed, if $H'$ is a level-$i$ cluster in $\hset$, and we partition it into a level-$(i+1)$ cluster $H''$ and a level-$i$ cluster $H'''$, then we are guaranteed that $|X\cap V(H'')|\leq 2d |X\cap V(H')|/\beta$, from Theorem~\ref{thm: general partition of solution}. Therefore, if $H'\in \hset$ is a level-$i$ cluster, then $|X\cap V(H')|\leq N/(\beta/2d)^i$. Therefore, the maximum level of a cluster is at most $\log N/\log (\beta/2d)$. 

Denote $L^*=\frac{\log n}{\log\left(\frac{\beta}{2d(n)}\right )}$. From Invariant \ref{prop: charge each edge}, throughout the algorithm, for every edge $e\in E^1$, $b(e)\leq \eta^{L^*}$ must hold. Once an edge is added to $E^b\cup E^g$, its budget does not change. Therefore, at the end of the algorithm, the budget of every edge in $ E^g\cup E^b$ is at most $\eta^{L^*}$. On the other hand, from Invariant \ref{prop: total budget}, at the end of the algorithm, the total budget of all edges in $E^1\cup E^g\cup E^b$ is at least $|E(H)|$. Therefore, at the end of the algorithm:

\[|E^g\cup E^b|\geq \frac{|E(H)|}{\eta^{L^*}}. \]


We now bound $\eta^{L^*}$. Recall that 
$\eta=2^8 \cdot d(n)\cdot \gamma\cdot \alpha(n)\cdot \log^4n$, 

$\beta>4(d(n))^2$. Then $L^*=\frac{\log n}{\log\left(\frac{\beta}{2d(n)}\right )}\geq \frac{\log n}{2\log \beta}$.



Need: $2^{\log \eta\cdot \log n/\log \beta}<2^{\log \beta}$. So: $\log \eta<\frac{(\log \beta)^2}{\log n}$.


So $\log \beta>\sqrt{\log(d(n)\gamma\alpha(n))\log n \log\log n}$

$\beta>2^{\sqrt{\log(d(n)\gamma\alpha(n))\cdot \log n\log \log n}}$

@@@@@@@@@@@@@@@@@@@@@@@
@@@@


Notice that, once an edge is added to $E_1$ or to $E_2$, its charge stops increasing. Therefore, the charge to every edge is at most $C=(2\eta)^{\log N/\log(\beta/2d)}$. On the other hand, the total charge to all edges of $E_1\cup E_2$, which is at most $C|E_1\cup E_2|$, is at least $|E(\tilde H)|$. Therefore, we get that $|E_1\cup E_2|\geq |E(\tilde H)|/C$. In order to prove that $|E_1\cup E_2|\geq |E(\tilde H)|/\beta$, it is now enough to prove that $C\leq \beta$. Substituting $\eta=16d\alpha \log^{3}A\log N$, we get that:

\[C\leq \eta^{\log N/\log(\beta/2d)}\leq (16d\alpha \log^{3}A\log N)^{\log N/\log(\beta/2d)}\leq (d\alpha^2)^{\log N/\log(\beta/2d)}\leq \beta,  \]

if we assume that $d<\sqrt{\beta}$, and $\alpha<2^{c\log^2\beta/\log N}/d$ for some small enough constant $c$.

\end{proof}



\iffalse
\subsection{Proof of Theorem~\ref{thm: general partition of solution}}
We use as subroutine the following theorem.



\begin{theorem}\label{thm: partition or solution for no instance}
	Assume that there is an efficient $\alpha$-approximation algorithm $\aset$ for \DS. Then
	there is an efficient randomized algorithm that, given a subgraph $H'=(X',Y',E')\subseteq H$ of the original constraint graph $H=H(\phi)$, and the corresponding instance $\phi'\subseteq \phi$ of the CSP, does one of the following:
	
	\begin{itemize}
		\item either computes a bad set $\tilde E\subseteq E'$ of constraints, with $|\hat E|\geq |E'|/(4\log^2N)$; or
		\item computes a solution $f:X\rightarrow A$ to $\phi'$ satisfying at least $|E(H')|/\beta^8$ constraints in expectation (that is, we certify that $H'$ is a good graph); or
		\item computes a subgraph $H''=(X'',Y'',E'')\subseteq H'$ of $H'$, with: $|X''|\leq 2d|X'|/\beta$; $|Y''|\leq 2d|Y'|/\beta$; and $|E''|\geq \frac{\vol(X''\cup Y'')}{16d\alpha \log^{3}A\log N}$, where $\vol(S)=\sum_{v\in S}d_{H'}(v)$. 
	\end{itemize} 
\end{theorem}


Before we prove the theorem, we complete the proof of  %It now remains to prove Theorem~\ref{thm: partition or solution for no instance}.
\fi

==> DkS_conditional-backup.tex <==
\section{Conditional Hardness of \DkS}
\label{sec: conditional}



\subsection{Low-Degree 2-CSP Conjecture}
We consider the \BCSP problem, that is defined as follows.
The input to the problem consists of two sets $X,Y$ of variables, together with an integer $A>1$. Every variable $z\in X\cup Y$ takes values in set $[A]=\set{1,\ldots,A}$. We are also given a collection $\cset$ of constraints, where each constraint $C(x,y)\in \cset$ is defined over a pair of variables $x\in X$ and $y\in Y$. For each such constraint, we are given a truth table that, for every pair of assignments $a$ to $x$ and $a'$ to $y$, specifies whether $(a,a')$ \emph{satisfy} constraint $C(x,y)$. %We denote an instance of 2-CSP by  $\iset=(X,Y,A,A',\cset,\set{G_C}_{C\in \cset})$.
The \emph{value} of the CSP is the largest fraction of constraints that can be simultaneously satisfied by an assignment to the variables.

We associate with each constraint $C=C(x,y)\in \cset$, a bipartite graph $G_C=(L,R,E)$, where $L=R=[A]$, and there is an edge $(a,a')$ in $E$ iff the assignments $a$ to $x$ and $a'$ to $y$ satisfy $C$. Notice that instance $\iset$ of the \BCSP problem is completely defined by $X,Y,A,\cset$, and the graphs in $\set{G_C}_{C\in \cset}$, so we will denote $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$.
The \emph{size} of instance $\iset$ is defined to be $\size(\iset)=|\cset|\cdot A^2+|X|+|Y|$.


Consider some instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP. We say that $\iset$ is a \emph{$d$-to-$d$ instance} if, for every constraint $C$, every vertex of graph $G_C=(L,R,E)$  has degree at most $d$.
%The \LDCSP is a special case of 2-CSP, where the input is restricted to $d$-to-$d'$ instances, where $d$ and $d'$ are typically subpolynomial functions in $\size(\iset)$.


Consider now some functions $d(n),s(n):\reals^+\rightarrow \reals^+$. We assume that, for all $n$, $d(n)\geq 1$ and $s(n)<1$.
In a $(d(n),s(n))$-\LDCSP problem, the input is an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP, such that, if we denote by $n=\size(\iset)$, then the instance is $d(n)$-to-$d(n)$. We say that $\iset$ is a  \yi, if there is some assignment to the variables of $X\cup Y$ that satisfies at least $|\cset|/2$ of the constraints, and we say that it is a \ni, if the largest number of constraints of $\cset$ that can be simultaneously satisfied by any assignment is at most $s(n)\cdot |\cset|$. Given an instance $\iset$ of $(d(n),s(n))$-\LDCSP problem, the goal is to distinguish between the case where $\iset$ is a \yi and the case where $\iset$ is a \ni. If $\iset$ is neither a \yi nor a \ni, the output of the algorithm can be arbitrary.
We now state our conjecture regarding hardness of $(d(n),s(n))$-\LDCSP.

\begin{conjecture}
	\label{conj: main1}
	There is a constant $0<\eps<1$, such that the $(d(n),s(n))$-\LDCSP problem is \NP-hard for $d(n)=2^{(\log n)^{\eps}}$ and $s(n)= 1/2^{8 (\log n)^{1/2+\eps}}$. 
\end{conjecture}


\begin{theorem}
	\label{thm: main_DkS}
	Assume that \Cref{conj: main} holds and that $\P\ne \NP$, there is no efficient approximation algorithm for \DkS problem that achieves approximation factor $2^{(\log N)^{\eps}}$, where $N$ is the number of vertices in the input graph.
\end{theorem}



%We prove the following conditional hardness result of \DkS.
%
%
%\subsection{Conditional Hardness of \DkS}
%\label{subsec: DkS cond hardness}

The remainder of this section is dedicated to proving \Cref{thm: main_DkS}. A central notion that we use is a \emph{constraint graph} that is associated with an instance $\iset$ of $2$-CSP. 



\paragraph{Constraint Graph.}

Let $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ be an instance of the \BCSP problem. 
The \emph{constraint graph} associated with instance $\iset$ is denoted by $H(\iset)$, and it is defined as follows.
The set of vertices of $H(\iset)$ is the union of two subsets: set $U=\set{v(x)\mid x\in X}$ of vertices representing the variables of $X$, and set $V=\set{v(y)\mid y\in Y}$ of vertices representing the variables of $Y$. For convenience, we will not distinguish between the vertices of $V$ and the variables of $X$, so we will identify each variable $x\in X$ with its corresponding vertex $v(x)$. Similarly, we will not distinguish between vertices of $U$ and variables of $Y$. The set of edges of $H(\iset)$ contains, for every constraint $C=C(x,y)\in \cset$, edge $e_C=(x,y)$. We say that edge $e_C$ \emph{represents} the constraint $C$.
Notice that, if $E'$ is a subset of edges of $H(\iset)$, then we can define a set $\Phi(E')\subseteq \cset$ of constraints that the edges of $E'$ represent, namely: $\Phi(E')=\set{C\in \cset\mid e_C\in E'}$.
Next, we define bad sets of constraints and bad collections of edges.

\begin{definition}[Bad Set of Constraints and Bad Collection of Edges]
Let $\cset'\subseteq \cset$ be a collection of constraints of an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP, and let $0<\gamma\leq 1$ be a parameter. We say that $\cset'$ is a \emph{$\gamma$-bad set of constraints} if the largest number of constraints of $\cset'$ that can be simultaneously satisfied by any assignment to the variables of $X\cup Y$ is at most $\frac{|\cset'|}{\gamma}$.
If $E'\subseteq E(H(\iset))$ is a set of edges of $H(\iset)$, whose corresponding set $\Phi(E')$ of constraints is $\gamma$-bad, then we say that $E'$ is a \emph{$\gamma$-bad collection of edges}.
\end{definition}


The next observation easily follows from the definition of a bad set of constraints.


\begin{observation}\label{obs: bad constraints}
	Let $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ be an instance of bipartite 2-CSP, let $0<\gamma\leq 1$ be a parameter, and let $\cset',\cset''\subseteq \cset$ be two disjoint sets of constraints that are both $\gamma$-bad. Then $\cset'\cup \cset''$ is also a $\gamma$-bad set of constraints.
\end{observation}


Next, we define good subsets of constraints and good subgraphs of the constraint graph $H(\iset)$.


\begin{definition}[Good Set of Constraints and Good Subgraphs of $H(\iset)$]
	Let $\cset'\subseteq \cset$ be a collection of constraints of an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP, and let $0<\beta\leq 1$ be a parameter. We say that $\cset'$ is a \emph{$\beta$-good set of constraints}, if there is an assigmnet to variables of $X\cup Y$ that satisfies at least  $\frac{|\cset'|}{\beta}$ constraints of $\cset'$.
	If $E'\subseteq E(H(\iset))$ is a set of edges of $H(\iset)$, whose corresponding set $\Phi(E')$ of constraints is $\beta$-good, then we say that $E'$ is a \emph{$\beta$-good collection of edges}. Lastly, if $H'\subseteq H(\iset)$ is a subgraph of the constraint graph, and the set $E(H')$ of edges is $\beta$-good, then we say that graph $H'$ is \emph{$\beta$-good}.
\end{definition}


The next observation easily follows from the definition of a good set of constraints.


\begin{observation}\label{obs: good constraints}
	Let $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ be an instance of bipartite 2-CSP, let $0<\beta\leq 1$ be a parameter, and let $H',H''$ be two subgraphs of $H(\iset)$ that are both $\beta$-good and disjoint in their edges. Then graph $H'\cup H''$ is also $\beta$-good.
\end{observation}

The observation follows from the fact that, since graphs $H',H''$ are disjoint in their vertices, if we let $\cset'=\Phi(E(H'))$, $\cset''=\Phi(E(H''))$ be the sets of constraints associated with the edge sets of both graphs, then the variables participating in the constraints of $\cset'$ are disjoint from the variables participating in the constraints of $\cset''$. 








\begin{theorem}\label{thm: a phase outer DkS}
		Assume that there exists an efficient $\alpha(N)$-approximation algorithm $\aset$ for the \DS problem, where $N$ is the number of vertices in the input graph. Then there is an efficient algorithm, whose input consists of an instance $\iset=(X,Y,A,\cset,\set{G_C}_{C\in \cset})$ of \BCSP and parameters $n$,  $\gamma,\beta\geq 1$, so that $\size(\iset)\leq n$,  $\beta \geq 2^{23}\gamma^3(\alpha(n))^3(\log n)^{12}$, and $\iset$ is a $d(n)$-to-$d(n)$ instance of \BCSP. The algorithm  returns a partition $(E_1,E_2,E_3)$ of $E(H(\iset))$, where $E_1$ is a $\gamma$-bad set of constraints, $E_2$ is a $\beta^3$-good set of constraints, and $|E_1\cup E_2|\geq \frac{|E(H(\iset))|}{\beta}$.
\end{theorem}





\newpage
\input{DKS-outer-thm}
\input{DKS-inner-thm}


We say that a set $\cset'\subseteq \cset$ of constraints is \emph{good} iff there is an assignment to the variables satisfying at least $|\cset'|/\beta^3$ consraints of $\cset'$. We say that a subgraph $H'\subseteq H$ of the constraint graph is good iff $E(H')$ is a good set of constraints.
%Notice that some constraint sets are neither good nor bad. 
The following observation is immediate.

\begin{observation}\label{obs: good and bad constraints under union}
If $\cset',\cset''$ are disjoint bad sets of constraints, then $\cset'\cup \cset''$ is a bad set of constraints. If $H',H''\subseteq H$ are good graphs that are disjoint in their vertices, then $H'\cup H''$ is a good graph.
\end{observation}

%Our reduction is iterative. We will iteratively consider sub-graphs $H'\subseteq H(\phi)$ of the original constraint graph. Each such subgraph $H'$ naturally defines a CSP $\phi'$, whose variables are the vertices of $H'$ and constraints are defined by its edges. We can then construct an assignment graph $G'=G(\phi')$ associated with the constraint graph $H'=(X',Y',E'')$. We then construct an instance $\iset(\phi')=(G(\phi'),k_1,k_2)$ of \DS, where $G(\phi')$ is the assignment graph corresponding to $\phi'$, $k_1=|X'|$, and $k_2=|Y'|$.


%We assume that there is an $\alpha$-approximation algorithm $\aset$ for \DS, for some $\alpha<\beta$, whose exact value we set later (notice that $\alpha$ may be a function of the size of $G$.) For now, it is sufficient to assume that $\alpha<\beta/(2^{20}\log^7A\log^2N)$, though in the end we'll make $\alpha$ much smaller. We will reach a contradiction by showing that  $\aset$ can be used to distinguish between the yes- and the no-instances of the CSP. The following theorem is central to the analysis of the resulting algorithm.
 

Let $\phi$ be the input CSP instance and let $H=H(\phi)$ be its constraint graph. Note that each subgraph $H'\subseteq H$ naturally defines a CSP $\phi'$, whose variables are the vertices of $H'$ and constraints are defined by its edges.
%
The main technical result of this section is the following lemma.

\begin{lemma}\label{thm: a phase}
Assume that there is an efficient $\alpha$-approximation algorithm $\aset$ for \DS. Then there is an efficient randomized algorithm that, given a subgraph $\tilde H=(\tilde X,\tilde Y,\tilde E)\subseteq H$ of the original constraint graph $H=H(\phi)$,  returns a partition $(E_1,E_2,E_3)$ of $\tilde E$, where $E_1$ is a bad set of constraints, $E_2$ is a good set of constraints, and $|E_1\cup E_2|\geq |\tilde E|/\beta$.
\end{lemma}
 
 
 \subsection{Proof of Theorem~\ref{thm: a phase}}
 The main tool in the proof is the following theorem.
 
 \begin{theorem}\label{thm: general partition of solution}
 	Assume that there is an efficient $\alpha$-approximation algorithm $\aset$ for \DS. Then
 	there is an efficient randomized algorithm that, given a subgraph $H'=(X',Y',E')\subseteq H$ of the original constraint graph $H=H(\phi)$,  returns a partition $(E_1,E_2)$ of $E'$, where $E_1$ is a bad set of constraints, and:
 	
 	\begin{itemize}
 		\item either the algorithm certifies that $E_2$ is a good set of constraints;
 		\item or the algorithm produces a subgraph $H''=(X'',Y'',E'')\subseteq H'$ with $E''\subseteq E_2$, such that: $|X''|\leq 2d|X'|/\beta$, $|Y''|\leq 2d|Y'|/\beta$ and $|E''|\geq \frac{|E_2^*|}{16d\alpha \log^{3}A\log N}$, where $E_2^*\subseteq E_2$ is the set of all edges of $E_2$, connecting vertices of $H''$ to vertices of $V(H')\setminus V(H'')$. %\mynote{intuitively, we cut the edges of $E_2^*$, and we charge them to the edges of $E''$}. 
 	\end{itemize} 
 \end{theorem}	
 
 

We provide the proof of Theorem~\ref{thm: general partition of solution} in the following section, after we complete the proof of Theorem~\ref{thm: a phase} using it.

 For convenience, we denote $\eta= 16d\alpha \log^{3}A\log N$. 

Throughout the algorithm, we maintain a bad subset $E_1\subseteq E(\tilde H)$ of constraints, a good subset $E_2\subseteq E(\tilde H)$ of constraints, a subset $E_0\subseteq E(\tilde H)$ of \emph{deleted constraints}, and a collection $\hset$ of vertex-disjoint subgraphs of $\tilde H$. Let $E_3=\bigcup_{H'\in \hset}E(H')$. We also assign, to every graph $H'\in \hset$ a \emph{level}. Each edge $e$ of $E_1\cup E_2\cup E_3$ is assigned a \emph{charge} (which changes throughout the algorithm). We ensure that the total charge of all edges in $E_1\cup E_2\cup E_3$ is at least $|E(\tilde H)$. We also ensure that the following invariantes hold.

\begin{properties}{I}
	\item  $E_1,E_2,E_3,E_0$ partition the edges of $E(\tilde H)$ into disjoint subsets.
	
	\item All graphs in $\hset$ are disjoint in their vertices. 
	
	\item If we denote by $H_1$ and $H_2$ the sub-graphs of $\tilde H$ induced by the edges of $E_1$ and $E_2$, respectively, then all graphs in $\hset$ are vertex-disjoint from both $H_1$ and $H_2$ (but we allow $H_1$ and $H_2$ to share vertices).
	
	\item If $H'\in \hset$ is a level-$i$ graph, then the charge to each of its edges is at most $\eta^i$.
\end{properties}

%Additionally, for accounting purposes, we assign to every graph of $\tilde H$ a \emph{level}, which is a non-negative integer.
When the algorithm starts, we set $E_1=E_2=E_0=\emptyset$, and $\hset$ contains a single graph $\tilde H$, which is a level-$0$ graph. Every edge $e\in E(\tilde H)$ is assigned a charge of $1$. The algorithm continues as long as $\hset\neq \emptyset$. In every iteration, we select an arbitrary graph $H'\in \tilde H$ and process it.

Consider now some graph $H'\in \hset$, and assume that it belongs to level $i$. In order to process $H'$, we apply Theorem~\ref{thm: general partition of solution} to it. Assume that we obtain a partition $(E_1',E_2')$ of $E(H')$. We consider two cases. First, if $E_2'$ is a good set of constraints, then we add the edges of $E_1'$ to $E_1$, the edges of $E_2'$ to $E_2$, and delete $H'$ from $\hset$. 

Assume now that the algorithm from Theorem~\ref{thm: general partition of solution} returns a subgraph $H''$ of $H'\setminus E'_1$. Let $V_1=V(H'')$ and $V_2=V(H')\setminus V_1$. Let $\tilde E=E(H'')$ and let $\tilde E'=E_{H'}(V_1,V_2)\setminus E_1'$. Finally, let $\tilde E''=E_{H'}(V_2)\setminus E_1'$. Notice that $\tilde E,\tilde E',\tilde E''$ and $E'_1$ partition the edges of $E(H')$. We add the edges of $E'_1$ to $E_1$ (recall that $E'_1$ is a bad set of constraints, and from Observation~\ref{obs: good and bad constraints under union}, so is $E'_1\cup E_1$. We also add the edges of $\tilde E'$ to $E_0$. We remove $H'$ from $\hset$, and add two new graphs to $\hset$ instead: 
graph $H''$, that belongs to level $(i+1)$, and graph $H'''$ that belongs to level $i$, whose vertex set is $V_2$, and edge set is $\tilde E''$.
Next, we update the charges of all edges. The charge of every edge in $E(H''')$ remains unchaged. We increase the charge to every edge in $E(H'')$, so that they can cover the charge of every edge in $\tilde E'$. Recall that, since $H'$ is a level-$i$ graph, the charge to every vertex of $H'$ is at most $(2\eta)^i$. Recall also that Theorem~\ref{thm: general partition of solution} guarantees that 
$|E(H'')|\geq |\tilde E'|/\eta$. Since every edge in $E(H'')\cup \tilde E'$ has a charge of at most $(2\eta)^i$, we can distribute the charges of the edges in $\tilde E'$ among the edges of $E(H'')$, so that every edge in $E(H'')$ gets an additional charge of at most $\eta\cdot (2\eta)^i$, and so the new charge of every edge in $E(H'')$ is at most $(2\eta)^{i+1}$, as required. We set the charge of every edge in $\tilde E'$ to $0$.

The algorithm terminates when $\hset=\emptyset$. Clearly, we obtain a partition $(E_1,E_2,E_0)$ of $E(\tilde H)$ into three subsets, where $E_1$ is a bad set of constraints and $E_2$ is a good set of constraints. It remains to show that $|E_1\cup E_2|\geq |E(\tilde H)|/\beta$.
We use the charging scheme in order to prove this.

We start by showing that the largest level of any cluster in $\hset$ is bounded by $\log N/\log (\beta/2d)$. Indeed, if $H'$ is a level-$i$ cluster in $\hset$, and we partition it into a level-$(i+1)$ cluster $H''$ and a level-$i$ cluster $H'''$, then we are guaranteed that $|X\cap V(H'')|\leq 2d |X\cap V(H')|/\beta$, from Theorem~\ref{thm: general partition of solution}. Therefore, if $H'\in \hset$ is a level-$i$ cluster, then $|X\cap V(H')|\leq N/(\beta/2d)^i$. Therefore, the maximum level of a cluster is at most $\log N/\log (\beta/2d)$. Notice that, once an edge is added to $E_1$ or to $E_2$, its charge stops increasing. Therefore, the charge to every edge is at most $C=(2\eta)^{\log N/\log(\beta/2d)}$. On the other hand, the total charge to all edges of $E_1\cup E_2$, which is at most $C|E_1\cup E_2|$, is at least $|E(\tilde H)|$. Therefore, we get that $|E_1\cup E_2|\geq |E(\tilde H)|/C$. In order to prove that $|E_1\cup E_2|\geq |E(\tilde H)|/\beta$, it is now enough to prove that $C\leq \beta$. Substituting $\eta=16d\alpha \log^{3}A\log N$, we get that:

\[C\leq \eta^{\log N/\log(\beta/2d)}\leq (16d\alpha \log^{3}A\log N)^{\log N/\log(\beta/2d)}\leq (d\alpha^2)^{\log N/\log(\beta/2d)}\leq \beta,  \]

if we assume that $d<\sqrt{\beta}$, and $\alpha<2^{c\log^2\beta/\log N}/d$ for some small enough constant $c$.
 
 
 
 
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 \iffalse
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %----------------
 %old stuff from here on
 %-----------------------------------------------------------------
 %-----------------------------------------------------------------
 %-----------------------------------------------------------------
 \subsection{Proof of Theorem~\ref{thm: general partition of solution}}
 	We use as subroutine the following theorem.
 
 \begin{theorem}\label{thm: partition or solution for no instance}
 	Assume that there is an efficient $\alpha$-approximation algorithm $\aset$ for \DS. Then
 	there is an efficient randomized algorithm that, given a subgraph $H'=(X',Y',E')\subseteq H$ of the original constraint graph $H=H(\phi)$, and the corresponding instance $\phi'\subseteq \phi$ of the CSP, does one of the following:
 	
 	\begin{itemize}
 		\item either computes a bad set $\tilde E\subseteq E'$ of constraints, with $|\hat E|\geq |E'|/(4\log^2N)$; or
 		\item computes a solution $f:X\rightarrow A$ to $\phi'$ satisfying at least $|E(H')|/\beta^8$ constraints in expectation (that is, we certify that $H'$ is a good graph); or
 		\item computes a subgraph $H''=(X'',Y'',E'')\subseteq H'$ of $H'$, with: $|X''|\leq 2d|X'|/\beta$; $|Y''|\leq 2d|Y'|/\beta$; and $|E''|\geq \frac{\vol(X''\cup Y'')}{16d\alpha \log^{3}A\log N}$, where $\vol(S)=\sum_{v\in S}d_{H'}(v)$. 
 	\end{itemize} 
 \end{theorem}


Before we prove the theorem, we complete the proof of Theorem~\ref{thm: general partition of solution} using it. The algorithm is iterative. We start with $E_1=\emptyset$ and $E_2=E''$, and then iterate. In every iteration, we apply Theorem~\ref{thm: partition or solution for no instance} to the current graph $H'$, which is obtained from the original graph $H'$, by removing all edges of $E_1$ from it. If the outcome is a bad set $\tilde E\subseteq E_2$ of constraints, then we move the constraints in $\tilde E$ from $E_2$ to $E_1$, delete them from $H'$, and continue to the next iteration. If the outcome is a certificate that the current graph $H'$ is a good graph, we terminate the algorithm with the partition $(E_1,E_2)$ of $E''$, where $E_1$ is a bad set of constraints, and $E_2$ is a good set of constraints. Otherwise, the algorithm computes a subgraph $H''$ of the current graph $H'$. It is easy to verify that this subgraph has all required properties. We terminate the algorithm, and return $E_1$, $E_2$ and $H''$. %It now remains to prove Theorem~\ref{thm: partition or solution for no instance}.


%\section{Proof of Theorem~\ref{thm: partition or solution for no instance}}

%-----------------------------------------------------------------
%-----------------------------------------------------------------
%-----------------------------------------------------------------
%\begin{proofof}{Theorem~\ref{thm: partition or solution for no instance}}

The remainder of this subsection is dedicated to the proof of \Cref{thm: partition or solution for no instance}.

Notice that we can assume that $|E(H')|\geq \beta^8\geq \alpha^2\log^8A$, since otherwise it is sufficient to satisfy one constraint.
%
In order to make the analysis  simpler, it helps if we first regularize the graph $H'$, by computing a ``nice'' subgraph $H''\subseteq H'$. We will then reduce $H''$ to an instance of \DS.


\begin{definition}
Let $H'$ be a subgraph of the original constraint graph $H$, and let $\hat H=(\hat X,\hat Y,\hat E)$ be a subgraph of $H'$. We say that $\hat H$ is a $(d_1,d_2)$-nice subgraph of $H'$, if the following hold:
	\begin{itemize}
		\item $|\hat E|\geq |\hat X|\cdot d_1/(2\log^2 N)$;
		\item For every vertex $x\in \hat X$, $d_1\leq \deg_{H'}(x)< 2d_1$ (and so $\deg_{\hat H}(x)< 2d_1$); 
		\item For every vertex $y\in \hat Y$, $d_2\leq \deg_{H'}(y)< 4d_2\log N$ and
			$d_2\leq \deg_{\hat H}(y)\leq 2d_2$.
	\end{itemize}
	We say that $\hat H$ is a \emph{nice} subgraph of $H'$ iff it is a $(d_1,d_2)$-nice subgraph of $H'$ for any $d_1,d_2$.
\end{definition}

\begin{claim}\label{claim: regularizing constraint graph}
	There is an efficient algorithm, that, given a subgraph $H'\subseteq H$, computes a nice sub-graph $\hat H\subseteq H'$, such that $|E(\hat H)|\geq |E(H')|/(4\log^2N)$.
\end{claim}

%Note that we lose an $O(\log^2N)$-fraction of the edges due to the regularization step. But since we are aiming to much bigger hardness of approximation factors this will not affect the calculations much.

\begin{proof}
	The proof follows standard regularization process. Assume that $H'=(X',Y',E')$. We group the vertices of $X'$ into at most $\log N$ groups, where vertex $x$ lies in group $q$ iff $2^q\leq \deg_{H'}(x)<2^{q+1}$; in this case, all edges incident to $x$ are also said to belong to group $q$. Clearly, there is some group $q$ that contains at least $|E(H')|/\log N$ edges. We denote $d_1=2^q$. We then discard from $H'$ all vertices of $X'$, except those lying in group $q$. Let $\tilde H$ be the resulting graph. Then for every vertex $x\in V(\tilde H)\cap X'$, $d_1\leq \deg_{\tilde H}(x)<2d_1$, and $|E(\tilde H)|\geq |E(H')|/\log N$. In the next step, we will discard some vertices from $Y'$, to obtain the final graph $\hat H$. Clearly, for every vertex $x\in V(\hat H)\cap X'$, $\deg_{\hat H}(x)<2d_1$ will continue to hold.
	
	
	In our second step, we consider the vertices $y\in Y'$ one-by-one. We say that a vertex $y\in Y'$ is \emph{bad} iff $\deg_{\tilde H}(y)<\deg_{H'}(y)/2\log N$. We discard all bad vertices of $Y'$ from graph $\tilde H$, obtaining a new graph $\tilde H'$. Notice that $\sum_{y\in Y'}\deg_{\tilde H}(y)\geq \sum_{y\in Y'}\deg_{H'}(y)/\log N$, since $|E(\tilde H)|\geq |E(H')|/\log N$. A simple accounting shows that $|E(\tilde H')|\geq |E(\tilde H)|/2\geq |E(H')|/2\log N$. (If $y$ is a bad vertex, then at most $\deg_{H'}(y)/(2\log N)$ edges that are incident to $y$ are lost in this step. So in total, this step loses at most $\sum_{y\in Y'}\deg_{H'}(y)/(2\log N)\leq |E(H')|/2\log N$ additional edges). 
	
	Lastly, we group the remaining vertices of $Y'$ exactly like in Step 1: that is, we partition all good vertices of $Y'$ into at most $\log N$ groups, where vertex $y$ lies in group $r$ iff $2^r\leq \deg_{\tilde H'}(y)<2^{r+1}$; in this case, all edges incident to $y$ are also said to belong to group $r$. Clearly, there is some group $r$ that contains at least $|E(\tilde H)|/\log N\geq |E(H')|/(2\log^2N)$ edges. We denote $d_2=2^r$. We then discard from $\tilde H'$ all vertices of $Y'$, except those lying in group $r$. Let $\hat H$ be the resulting graph. Then for every vertex $y\in V(\hat H)\cap Y'$, $d_2\leq \deg_{\hat H}(y)<2d_2$, and, since only good vertices of $Y'$ remain in $\hat H$, $d_2\leq\deg_{H'}(y)\leq 4d_2\log N$. Moreover, $|E(\hat H)|\geq |E(\tilde H)|/\log N\geq |E(H')|/2\log^2 N$, and in particular, $|E(\hat H)|\geq \sum_{v\in X'\cap V(\hat H)}\deg_{H'}(v)/\log^2N\geq d_1|X'\cap V(\hat H)|/2\log^2N$. %Notice however that for vertices $x\in V(H'')\cap X'$, we are only guaranteed that $\deg_{H''}(x)<2d_1$, as some of the edges incident to $x$ may have been deleted in the last step. However, since $|E(\tilde H)|\geq |X'\cap V(\tilde H)|\cdot d_1=|X'\cap V(H'')|\cdot d_1$, we get that $|E(H'')|\geq |X'\cap V(H'')|\cdot d_1/\log N$.
\end{proof}


Our algorthm starts by applying Claim~\ref{claim: regularizing constraint graph} to graph $H'$, to obtain a new graph $\hat H=(\hat X,\hat Y,\hat E)$, that is $(d_1,d_2)$-nice, for some $d_1,d_2$, such that $|E(\hat H)|\geq |E(H')|/(4\log^2N)$. Let $\hat \phi\subseteq \phi$ be the instance of CSP that corresponds to the constraint graph $\hat H$.

\paragraph{Assignment Graph.}
The assignment graph, $G=G(\phi)$ is defined as follows. The graph is a bipartite graph $G=(U,V,E)$.
%
For every variable $z\in X\cup Y$, we define a set $S(z)=\set{v(z,a)\mid 1\leq a\leq A}$ of vertices. We refer to $S(z)$ as the \emph{cloud of $z$}. We then set $U=\bigcup_{x\in X}S(x)$, and $V=\bigcup_{y\in Y}S(y)$.
%
In order to define the edges, 
consider any constraint $C=(x,y)$. We define a set $E(C)$ of at most $dA$ edges corresponding to $C$, as follows: we add an edge between $v(x,a)$ and $v(y,a')$ to $E(C)$ iff $a$ and $a'$ satisfy the constraint $C$. Therefore, every vertex of $S(x)\cup S(y)$ is incident to at most $d$ edges of $E(C)$.
We then let $E(G)=\bigcup_{C\in \cset}E(C)$.



We then construct an assignment graph $G=G(\hat \phi)$ for $\hat \phi$, which becomes an input to the \DS problem, with parameters $k_1=|\hat X|$ and $k_2=|\hat Y|$. Notice that, if $\phi$ is a \yi, then there is a solution to the resulting instance of the \DS problem, of value $|\hat E|$: the solution uses the satisfying assignment $f$ to all variables of $\hat X\cup \hat Y$ to define subsets $\hat X'=\set{(x,a)\mid x\in \hat X; f(x)=a}$ and $\hat Y'=\set{(y,a')\mid y\in \hat Y; f(y)=a'}$ of vertices. Since the assignments in $f$ satisfy all constraints of $\hat \phi$, $|E_{G}(\hat X',\hat Y')|=|E(\hat H)|$.

In our next step, we apply the approximation algorithm $\aset$ to $\DS$ to the resulting instance $(G,k_1,k_2)$ of \DS. If the value of the resulting solution is below $|E(\hat H)|/\alpha$, then, from the above discussion, $\phi$ must be a \ni. We terminate the algorithm and report ``\ni''. Therefore, we assume from now on that algorithm $\aset$ has returned a solution $G'\subseteq G$ to the DS instance, of value at least $|E(\hat H)|/\alpha$.


Intuitively, we would like to ensure that (i) for all $x\in \hat X$ with $S(X)\cap V(G')\neq \emptyset$, $|S(X)\cap V(G')|$ have roughly the same cardinalities; (ii) for all $y\in \hat Y$ with $S(Y)\cap V(G')\neq \emptyset$, $|S(Y)\cap V(G')|$ have roughly the same cardinalities; and 
(iii) for all $C\in E(\hat H)$ with $E(C)\cap E(G')\neq \emptyset$, $|E(C)\cap E(G')$ have roughly the same cardinalities.
Our next step is to regularize this solution, using the following claim.


\begin{claim}\label{claim: regularization}
	There is an efficient algorithm to compute a subgraph $G''\subseteq G'$, subsets $X^*\subseteq \hat X$, $Y^*\subseteq \hat Y$ of variables, and $E^*\subseteq E_{\hat H}(X^*,Y^*)$ of constraints, such that, if we denote, for each variable $z\in X^*\cup Y^*$,  $S'(z)= S(z)\cap V(G'')$, and for each constraint $C\in E^*$, $E'(C)= E(C)\cap E(G'')$, then for some integers $q,q',h$:
	
	\begin{itemize}
		\item for all $x\in X^*$, $2^q\leq |S'(x)|< 2^{q+1}$;
		\item for all $y\in Y^*$, $2^{q'}\leq |S'(y)|< 2^{q'+1}$;
		\item for all $C\in E^*$, $2^r\leq |E'(C)|<2^{r+1}$;  and
%		\item if $C=(x,y)\in E^*$, and $e=((x,a),(y,a'))\in E'(C)$, then $(x,a)\in S'(x)$ and $(y,a')\in S'(y)$; and
		\item $|E^*|\cdot 2^r\geq |\hat E|/(2\alpha\log^3A)$.
	\end{itemize}
\end{claim}

\begin{proof}
	The proof follows a standard regularization procedure. Let $E_0=E(G')$, so that $|E_0|\geq |E(\hat H)|/\alpha$.
	
	Our first step regularizes the variables of $\hat X$. We group the variables of $\hat X$ into $\log A$ groups, where variable $x\in \hat X$ lies in group $q$ iff $2^q\leq |S(x)\cap V(G')|<2^{q+1}$; if $x$ lies in group $q$, then all edges of $E_0$ that are incident to vertices of $S(x)$ also lie in group $q$. Clearly, some group $q$ contains at least $|E_0|/\log A$ edges of $E_0$. We let $X^*\subseteq \hat X$ be the set of variables that belong to group $q$, and for each such variable $x\in X^*$, let $S'(x)=S(x)\cap V(G')$. Let $E_1\subseteq E_0$ be the set of edges that belong to group $q$ (these are the edges of $G'$ that are incident to vertices of $\bigcup_{x\in X^*}S'(x)$.). Note that $|E_1|\geq |E_0|/\log A$.
	
	Our second step is to regularize the variables of $\hat Y$, exactly as before. We group the variables of $\hat Y$ into $\log A$ groups, where variable $y\in \hat Y$ lies in group $q'$ iff $2^{q'}\leq |S(x)\cap V(G')|<2^{q'+1}$; if $y$ lies in group $q'$, then all edges of $E_1$ that are incident to vertices of $S(y)$ also lie in group $q'$. Clearly, some group $q'$ contains at least $|E_1|/\log A\geq |E_0|/\log^2A$ edges of $E_1$. We let $Y^*\subseteq \hat Y$ be the set of variables that belong to group $q'$, and for each variable $y\in Y^*$, we let $S'(y)=S(Y)\cap V(G')$. We also let $E_2\subseteq E_1$ be the set of edges that belong to group $q'$ (these are the edges of $G'$ with one endpoint in $\bigcup_{x\in X^*}S'(x)$, and another endpoint in $\bigcup_{y\in Y^*}S'(y)$.). Note that $|E_2|\geq |E_0|/\log^2A$.
	
	Our third and last step is to regularize the constraints. We group all constraints $C\in \hat E$ into $\log A$ groups, where constraint $C\in \hat E$ belongs to group $r$ iff $2^r\leq |E(C)\cap E_2|<2^{r+1}$; we then say that the edges of $E(C)\cap E_2$ belong to group $r$ as well. Clearly, some group $r$ contains at least $|E_2|/\log A\geq |E_0|/\log^3A$ edges. We then let $E^*\subseteq \hat E$ be the set of all constraints of group $r$, and we let $E_3\subseteq E_2$ be the set of all edges of group $r$. For each constraint $C\in E^*$, we let $E'(C)=E(C)\cap E_3$ be the corresponding set of edges, so that $2^r\leq |E'(C)|<2^{r+1}$. Notice that $|E^*|\cdot 2^r\geq |E_3|/2\geq |\hat E|/(2\alpha\log^3A)$.
\end{proof}


It will be convenient for us to establish several bounds on $|E^*|$, $2^r$, $2^q$, and $2^{q'}$.

\begin{observation}
$|X^*|\leq |\hat X|/2^q$; $|Y^*|\leq |\hat Y|/2^{q'}$;  $|E^*|\leq 2d_1|X^*|\leq 2d_1|\hat X|/2^q$; and $|E^*|\leq 2d_2|Y^*|\leq 2d_1|\hat Y|/2^{q'}$.
\end{observation}

\begin{proof}
	Recall that $G'$ contained at most $k_1=|\hat X|$ vertices of $\bigcup_{x\in \hat X}S(x)$. Since, for every vertex $x\in X^*$, $S'(x)\subseteq G'$, we get that $|X^*|\leq |\hat X|/2^q$. Similarly, $|Y^*|\leq |\hat Y|/2^{q'}$. 
	
	Since every vertex of $\hat X$ is incident to at most $2d_1$ constraints in $\hat H$, we get the third inequality. The fourth inequality is obtained similarly.
\end{proof}

Next, we show that $2^q,2^{q'}$ are close to $2^r$.

\begin{corollary}\label{cor: q q' and r}
$2^r/2d\leq 2^{q}\leq 2^{2r+2}\alpha \log N\log^3A$, and $2^r/2d\leq 2^{q'}\leq 2^{2r+4}\alpha\log^3A$.
\end{corollary}

\begin{proof}
	The inequalities $2^r\leq 2^qd/2$ and $2^r\leq 2^{q'}d/2$ are immediate, because for every every constraint $C=(x,y)\in E^*$, every vertex $v(x,a)\in S'(x)$ may contribute at most $d$ edges to $E'(C)$, and there are at most $2^{q+1}$ such vertices, while $|E'(C)|\geq 2^r$. similarly, every vertex $v(y,a')\in S'(y)$ may contribute at most $d$ edges to $E'(C)$, and there are at most $2^{q'+1}$ such vertices.
	We now prove the other direction.
	
Recall that $|E^*|\cdot 2^r\geq |\hat E|/(2\alpha\log^3A)$, and $|\hat E|\geq d_2|\hat Y|$, so altogether:

\begin{equation}
|E^*|\geq \frac{d_2|\hat Y|}{2^{r+1}\alpha\log^3A}.  \label{eq2}
\end{equation} 

On the other hand, every variable $y\in Y^*$ contributes at most $2d_2\cdot 2^r$ edges to $E^*$, and $|Y^*|\leq |\hat Y|/2^{q'}$. Therefore:
$|E^*|\leq \frac{2|\hat Y|d_2 2^r}{2^{q'}}$.
%
Combining the two inequalities together, we get that: $2^{q'}\leq 2^{2r+2}\alpha \log^3A$.

Similarly, $|E^*|\cdot 2^r\geq |\hat E|/(2\alpha\log^3A)$, and $|\hat E|\geq d_1|\hat X|/(4\log N)$, so altogether: 


\begin{equation}
|E^*|\geq \frac{d_1|\hat X|}{2^{r+3}\alpha\log N\log^3A}.  \label{eq1}
\end{equation}

On the other hand, every variable $x\in X^*$ contributes at most $2d_1\cdot 2^r$ edges to $E^*$, and $|X^*|\leq |\hat X|/2^{q}$. Therefore:
$|E^*|\leq \frac{2|\hat X|d_1 2^r}{2^{q}}$.
Combining the two inequalities together, we get that: $2^{q}\leq 2^{2r+4}\alpha \log N\log^3A$.
\end{proof}

We now consider two cases, based on whether $2^r\leq \beta$ holds or not.


\paragraph{Case 1: $2^r\leq \beta$.} In this case, we compute an assignment to the variables of $\hat X\cup \hat Y$ that satisfies a large fraction of the constraints in $E'$. In order to compute the assignment, every variable $x\in X^*$ chooses one of its at most $2^{q+1}$ assignments in $S'(x)$ uniformly at random, and similarly, every variable $y\in Y^*$ chooses one of its assignments in $S'(y)$ uniformly at random. We now show that this assignment satisfies many constraints. In order to do so, we show that (i) $|E^*|$ is quite large; and (ii) every constraint in $E^*$ is satisfied with a high enough probability. In order to show (i), recall that:

\[|E^*|\cdot 2^r\geq \frac{|\hat E|}{2\alpha\log^3A} \geq \frac{|E(H')|}{8\alpha\log^3A\log^2N}. \]

Therefore:

\[|E^*|\geq \frac{|E(H')|}{8\cdot 2^r\alpha\log^3A\log^2N}\geq\frac{|E(H')|}{8\cdot \beta\alpha\log^3A\log^2N}\geq\frac{|E(H')|}{\beta^2}.\]

On the other hand, the probability that a constraint $C\in E^*$ is satisfied is at least:

\[\frac{2^r}{2^{q+1}\cdot 2^{q'+1}}\geq \frac{2^r}{2^{4r+6}\alpha^2 \log N\log^6A}\geq \frac{1}{2^{3r+6}\alpha^2\log N\log^6A}\geq \frac{1}{\beta^4}.\]
	
	Therefore, the expected number of constraints we satisfy is at least $\frac{|E(H')|}{\beta^6}$.
	
	
	\paragraph{Case 2: $2^r>\beta$.}
In this case, we return a sub-graph $H''=(X'',Y'',E'')\subseteq H'$, defined as follows: $X''=X^*$; $Y''= Y^*$; and $E''=E^*$. 
Since $|X^*|\leq |\hat X|/2^q\leq 2d|X'|/2^r$, we get that $|X''|\leq 2d|X'|/\beta$. Similarly, since $|Y^*|\leq |\hat Y|/2^{q'}\leq 2d|Y'|/2^r$, we get that $|Y''|\leq 2d|Y'|/\beta$. It now only remains to show that:

\[|E''|\geq \frac{\vol(X''\cup Y'')}{16d\alpha\log^{3}A\log N},\]

 where $\vol(S)$ for a set $S$ of vertices of $H'$ is the sum of the degrees of these vertices in $H'$, that is, $\vol(S)=\sum_{v\in S}d_{H'}(v)$. 

Recall that, from Equation~\ref{eq1}, $|E^*|\geq \frac{d_1|\hat X|}{2^{r+1}\alpha\log N\log^3A}$, and, since $2^q\geq 2^r/2d$, $|E^*|\geq \frac{d_1|X'|}{2^{q+2}d\alpha\log N\log^3A}$. At the same time, $\vol(X'')\leq 2d_1|X^*|\leq 2d_1|X'|/2^{q}$. Therefore, $|E^*|\geq \vol(X'')/(8d\alpha\log N\log^3A)$. 

Similarly,  $|E^*|\geq \frac{d_2|\hat Y|}{2^{r+1}\alpha\log^3A}$ from Equation~\ref{eq2}, and, since $2^{q'}\geq 2^r/2d$, $|E^*|\geq \frac{d_2|Y'|}{2^{q'+2}d\alpha\log^3A}$. At the same time, $\vol(Y'')\leq 4d_2|Y^*|\log N\leq 4d_2|Y'|\log N/2^{q'}$. Therefore, $|E^*|\geq \vol(Y'')/(16d\alpha\log N\log^3A)$. Altogether, 

\[ |E^*|\geq \frac{\vol(X''\cup Y'')}{16d\alpha\log N\log^3A}.  \]


%\end{proofof}
\fi
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------
%----------------

==> DkS_to_DkCWGP.tex <==
\section{Reductions from \DkC and \WGP to \DkS}
\label{sec: DkC and WGP to DkS}

In this section we prove the following theorem.

\begin{theorem}
\label{thm: alg_DkS gives alg_DkC}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. 
If there exists an efficient algorithm that, given an instance of \DkS whose graph contains $n$ vertices, computes an $\alpha(n)$-approximate solution, then
\begin{itemize}
\item there exists an efficient randomized algorithm that, given an instance \DkC whose graph contains $N$ vertices, with high probability computes an $O(\alpha(N)\cdot\poly\log N)$-approximate solution; and
\item there exists an efficient randomized algorithm that, given an instance of \WGP whose graph contains $N$ vertices, with high probability computes an $O(\alpha(N)\cdot\poly\log N)$-approximate solution.
\end{itemize}
\end{theorem}


The proofs of \Cref{thm: alg_DkS gives alg_DkC} are divided into three parts. 
First, from \Cref{lem: DkS and Dk1k2S}, an $\alpha(n)$-approximation algorithm for \DkS gives an $O(\alpha(N^2))$-approximation algorithm for \DBS. 
We then show in \Cref{sec: densest k_1 k_2 gives DkC and WGP} that an $O(\alpha(n))$-approximation algorithm for the Densest $(k_1,k_2)$-Subgraph problem gives $O(\alpha(n)\cdot\poly\log n)$-approximation algorithms for \DkC and \WGP on bipartite graphs. Finally, we show in \Cref{sec: bipartite to general} that $O(\alpha(n)\cdot \poly\log n)$-approximation algorithms for \DkC and \WGP on bipartite graphs give $O(\alpha(n)\cdot\poly\log n)$-approximation algorithms for \DkC and \WGP on general graphs. The combination of \Cref{thm: alg_DkS gives alg_DkC} and the results in \Cref{sec: densest k_1 k_2 gives DkC and WGP} and \ref{sec: bipartite to general} completes the proofs of \Cref{thm: alg_DkS gives alg_DkC} and \Cref{thm: alg_DkS gives alg_WGP}.













\subsection{From \DkC and \WGP on bipartite graphs to Densest $(k_1,k_2)$-Subgraph}
\label{sec: densest k_1 k_2 gives DkC and WGP}

In this subsection, we prove the following lemmas.

\begin{lemma}
\label{lem: alg_Dk1k2 gives alg_DkC}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. If there exists an efficient $\alpha(n)$-approximation algorithm for the Densest $(k_1,k_2)$-Subgraph problem, then there exists an efficient $O(\alpha(n)\log^2 n)$-approximation algorithm for \DkC on bipartite graphs.
\end{lemma}

\begin{lemma}
\label{lem: alg_Dk1k2 gives alg_WGP}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. If there exists an efficient $\alpha(n)$-approximation algorithm for the Densest $(k_1,k_2)$-Subgraph problem, then there exists an efficient $O(\alpha(n)\log^2 n)$-approximation algorithm for \DkC on bipartite graphs.
\end{lemma}

We only provide the proof of \Cref{lem: alg_Dk1k2 gives alg_DkC} here. The proof of \Cref{lem: alg_Dk1k2 gives alg_WGP} is very similar to the proof of \Cref{lem: alg_Dk1k2 gives alg_DkC}, and is deferred to \Cref{apd: Proof of alg_Dk1k2 gives alg_WGP}.

Let $\pcl(G,k)$ be the input instance of \DkC, where $G=(A,B,E)$ is a bipartite graph. 
We denote $|A\cup B|=n$ and assume that $\log_2 n$ is an integer (note that this can be guaranteed by adding to $G$ isolated vertices, at most doubling the number of vertices in $G$).
We denote $V=A\cup B$. We consider the following LP, whose variables are $\set{x_S}_{S\subseteq V: |S|\le k}$.
%
\begin{eqnarray*}
	\mbox{(LP-1)}	&\text{maximize } \sum_{S\subseteq V: |S|\le k} x_S\cdot |E_G(S)|\\
	\mbox{s.t.}&&\\
	&\sum_{|S|\le k: v\in S} x_S\leq 1 &\forall v\in V\\
	&\sum_{|S|\le k}x_S \leq \ceil{\frac n k}\\
	&x_S\geq 0&\forall S\subseteq V
\end{eqnarray*}
%
It is easy to verify that $\opt(\textnormal{LP-1})\ge \optcl(G,k)$, since for every solution $\sset$ to instance $\pcl(G,k)$, we can construct a feasible solution to (LP-1) where $x_S=1$ for every $S\in \sset$ and $x_S=0$ for every $S\notin \sset$, whose value in (LP-1) is exactly $|E_G(\sset)|$.

We consider the following LP whose variables are $z$ and $\set{y_v}_{v\in V}$, that is the dual of (LP-1).
%
\begin{eqnarray*}
	\mbox{(LP-2)}	&\text{minimize } \ceil{\frac{n}{k}}\cdot z+\sum_{v\in V} y_v\\
	\mbox{s.t.}&&\\
	& z+\sum_{v\in S} y_v\geq |E_G(S)| &\forall S\subseteq V: |S|\subseteq k\\
	&z\ge 0\\
	&y_v\geq 0&\forall v\in V
\end{eqnarray*}
%
It is folklore that, in order to efficiently compute a $\beta$-approximation solution to (LP-1), it suffices to construct an efficient $\beta$-approximate separation oracle for (LP-2), where a $\beta$-approximate separation oracle for (LP-2) is an algorithm that takes as input a real number $z$ and a set $\set{y_v}_{v\in V}$ of real numbers, and either correctly reports that $z+\sum_{v\in V} y_v\geq |E_G(S)|/\beta$ holds for all $S$, or find a set $S\subseteq V, |S|\le k$ such that $z+\sum_{v\in V} y_v< |E_G(S)|$ (that corresponds to a violating constraint in (LP-2)). We prove the following claim.

\begin{claim}
\label{clm: separation oracle}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. If there is an efficient $\alpha(n)$-approximation algorithm for the Densest $(k_1,k_2)$-Subgraph problem, then there exists an efficient $O(\alpha(n)\log^2 n)$-approximate separation oracle for (LP-2).
\end{claim}

\begin{proof}
Let $(z,\set{y_v}_{v\in V})$ be the input real numbers.
Note that $V=A\cup B$. For each integer $-3\log n\le t\le 2\log n$, we define $A_t=\set{v\in A\mid 2^t\le y_v <2^{t+1}}$ and $B_t=\set{v\in B\mid 2^t\le y_v <2^{t+1}}$, and we denote $A_{-3\log n-1}=A\setminus \big(\bigcup_{-3\log n\le t\le 2\log n}A_t\big)$ and $B_{-3\log n-1}=B\setminus \big(\bigcup_{-3\log n\le t\le 2\log n}B_t\big)$, so for all vertices $v\in A_{-3\log n-1}\cup B_{-3\log n-1}$, we have $y_v<1/n^3$.

\tnote{getting rid of small coordinates in the construction of separation oracle}

We say that a pair $(k_1,k_2)$ of integers are \emph{eligible}, iff $k_1,k_2\ge 0$ and $k_1+k_2\le k$. For each eligible pair $(k_1,k_2)$, and for each pair $-3\log n-1\le i,j\le 2\log n$, we apply the $\alpha(n)$-approximation algorithm for the Densest $(k_1,k_2)$-Subgraph problem to instance $\pdks(G[A_i, B_j],k_1,k_2)$, and let $S^{k_1,k_2}_{i,j}$ be the solution we get, so $|E(S^{k_1,k_2}_{i,j})|\ge \optdks(G[A_i, B_j],k_1,k_2)/\alpha(n)$. We then check if the constraint
\[z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v\geq |E_G(S^{k_1,k_2}_{i,j})|\] 
is satisfied (note that such a constraint indeed exists in (LP-2) since $|S^{k_1,k_2}_{i,j}|= k_1+k_2\le k$). If not, then we return it as the violating constraint.
If for all eligible pairs $(k_1, k_2)$ and all integer pairs $-3\log n-1\le i,j\le 2\log n$, the above constraint is satisfied, then the algorithm reports that, for all sets $S\subseteq V$ with $|S|\le k$, $z+\sum_{v\in V} y_v\geq |E_G(S)|/\beta$ holds for $\beta=100\alpha(n)\log^2 n$.

\tnote{separation oracle: not we, but "the algorithm" reports}

It remains to show that the above algorithm is indeed a $\beta$-approximate separation oracle. On the one hand, it is clear that if we return a violated constraint, then indeed the constraint is violated by the solution $(z,\set{y_v}_{v\in V})$. On the other hand, consider the case where for all eligible pairs and all pairs $-3\log n-1\le i,j\le 2\log n$, the above constraint is satisfied. Let $S$ be any set such that $S\subseteq V$ and $|S|\le k$.
Denote $S'=S\cap \big(\bigcup_{-3\log n\le i\le 2\log n}A_i\cup B_i\big)$ and $S''=S\setminus S'$. Consider now any pair $-3\log n\le i,j\le 2\log n$ and denote $p_i=|S\cap A_{i}|$ and $q_j=|S\cap B_{j}|$. Since $|S|\le k$, we get that $|S\cap A_{i}|+|S\cap B_{j}|\le k$, so $(p_i,q_j)$ is an eligible pair. Recall that we have applied the $\alpha(n)$-approximation algorithm to instance $\pdks(G[A_i, B_j],p_i,q_j)$, and certified that
\[z+\sum_{v\in S^{p_i,q_j}_{i,j}} y_v\geq |E_G(S^{p_i,q_j}_{i,j})|\ge \frac{\optdks(G[A_i, B_j],p_i,q_j)}{\alpha(n)}\ge \frac{|E(S\cap A_i, S\cap B_j)|}{\alpha(n)}.\]
Note that $|S^{p_i,q_j}_{i,j}\cap A_i|=p_i=|S\cap A_i|$, $|S^{p_i,q_j}_{i,j}\cap B_j|=y_i=|S\cap B_j|$. Also note that the $y_v$ values for all vertices in $A_i$ are within factor $2$ from each other, and so are the $y_v$ values for all vertices in $B_j$. It follows that
\[\sum_{v\in (S\cap A_i)}y_v\ge \frac{1}{2}\cdot\bigg(\sum_{v\in S^{p_i,q_j}_{i,j}\cap A_i} y_v\bigg); \text{ and } \sum_{v\in (S\cap B_j)}y_v\ge \frac{1}{2}\cdot\bigg(\sum_{v\in S^{p_i,q_j}_{i,j}\cap B_j} y_v\bigg),\]
and so 
\[ z+\sum_{v\in S\cap (A_i\cup B_j)} y_v \ge \frac{|E(S\cap A_i, S\cap B_j)|}{2\alpha(n)}.\]
%
\tnote{replace $-3\log n$ and $2\log n$ with symbols $z, z'$}

Therefore, summing over all pairs $-3\log n\le i,j\le 2\log n$, we get that
\begin{equation}
\label{eq1}
30z\log^2 n+\sum_{v\in S'} y_v\geq  \sum_{-3\log n\le i,j\le 2\log n}\frac{|E(S\cap A_i, S\cap B_j)|}{2\alpha(n)}\ge \frac{|E(S')|}{2\alpha(n)}.
\end{equation}
%
Finally, we consider sets $A'=A_{-3\log n-1}$ and $B'=B_{-3\log n-1}$. Since $y_v<1/n^3$ for all $v\in A'\cup B'$, we get that $\sum_{v\in (A'\cup B')}y_v\le 1/n^2$.
For every $-3\log n\le i\le 2\log n$, we have certified that
\[z+\sum_{v\in S^{p_i,q_{-3\log n-1}}_{i,-3\log n-1}} y_v\geq \frac{|E(S\cap A_i, S\cap B')|}{\alpha(n)},\quad\text{and }\quad z+\sum_{v\in S^{p_{-3\log n-1},q_j}_{2\log n-1,j}} y_v\geq \frac{|E(S\cap A', S\cap B_i)|}{\alpha(n)},\]
from which we can deduce (using similar arguments) that 
\begin{equation}
\label{eq2}
z+\sum_{v\in S\cap (A_i\cup B')}y_v\ge \frac{|E(S\cap A_i, S\cap B')|}{2\alpha(n)}-\frac{1}{n^2},\quad\text{and}\quad z+\sum_{v\in S\cap (A'\cup B_i)} y_v\geq \frac{|E(S\cap A', S\cap B_i)|}{2\alpha(n)}-\frac{1}{n^2}.
\end{equation} 
%
Note that we have also certified that
\[
z+\sum_{v\in (A'\cup B')}y_v\ge \frac{|E(S\cap A', S\cap B')|}{\alpha(n)},\]
so
\begin{equation}
\label{eq3}
z\ge \frac{|E(S\cap A', S\cap B')|}{\alpha(n)}-\frac{1}{n^2}.
\end{equation}

Combining inequalities \ref{eq1}, \ref{eq2}, and \ref{eq3}, we get that
\[31\log^2 n\cdot z+\sum_{v\in S} y_v\geq   \frac{|E(S)|}{2\alpha(n)}-\frac{12\log n}{n^2}.\]
Since $\alpha(n)=o(n^2/\log n)$, we get that $31\log^2 n\cdot z+\sum_{v\in S} y_v\geq  |E(S)|/3\alpha(n)$, which implies that $ z+\sum_{v\in S} y_v\geq  |E(S)|/(100\log^2 n\cdot\alpha(n))$, so our claim is correct. 
\end{proof}



We compute a solution to instance $\pcl(G,k)$ as follows. We first compute an $O(\alpha(n)\log^2 n)$-approximate solution $x^*$ to (LP-1) using the separation oracle in \Cref{clm: separation oracle}, so $x^*$ satisfies all constraints in (LP-1), and 
\[\sum_{|S|\le k}x^*_S\cdot |E(S)|\ge \Omega\bigg(\frac{\opt(\textnormal{LP-1})}{\alpha(n)\log^2 n}\bigg)\ge 
\Omega\bigg(\frac{\optcl(G,k)}{\alpha(n)\log^2 n}\bigg).\]
We then let $\sset$ contain, for each $S\subseteq V$ such that $|S|\le k$, the set $S$ independently with probability $x^*_S$, so clearly $\expect{|E(\sset)|}=\sum_{|S|\le k}x^*_S\cdot |E(S)|\ge\Omega(\optcl(G,k)/(\alpha(n)\log^2 n))$.
We use the following observation.

\begin{observation}
\label{obs: bad event}
With probability $1-O(n^{-3})$, each vertex appears in at most $4\log n$ sets in $\sset$, and $|\sset|\le 4n\log n/k$.
\end{observation}
\begin{proof}
Let $v\in V$ be a vertex and consider the constraint $\sum_{|S|\le k: v\in S} x_S\leq 1$ in (LP-1). For each set $S$, we denote by $Y_S$ the indicator variable of the event that the set $S$ is contained in $\sset$, so each $Y_i$ takes value from $\set{0,1}$ and $\sum_{S}\expect{Y_S}=\sum_S x^*_S\le 1$. From the Chernoff Bound (\Cref{lem: Chernoff}), we get that $\Pr[\sum_{S}Y_S\ge 4\log n]\le \exp(-4\log n)=O(1/n^4)$.
Then from the union bound over all vertices in $V$, the probability that some vertex appears in more than $4\log n$ sets in $\sset$ is at most $O(n^{-3})$.
From similar arguments on the constraint $\sum_{|S|\le k}x_S \leq \ceil{\frac n k}$ in (LP-1), we can show that the probability that $\sset$ contains more than $4n\log n/k$ sets is at most $O(n^{-3})$.
\end{proof}

We say that the event $\event$ happens iff either there exists a vertex that appears in more than $4\log n$ sets in $\sset$ or $|\sset|> 4n\log n/k$. From \Cref{obs: bad event}, $\Pr[\event]=O(n^{-3})$.

We construct a collection $\sset'$ based on $\sset$ as follows. For each $v\in V$, if the sets in $\sset$ that contain $v$ are $S_1,\ldots,S_t$, then we independently pick an integer $i$ uniformly at random from $[t]$, and delete vertex $v$ from all sets $S_1,\ldots,S_{i-1}, S_{i+1},\ldots,S_t$. Let $\sset'$ be the obtain collection of sets after processing all vertices in $V$ in this way. Since the sets in $\sset$ have size at most $k$, from the construction of $\sset'$ the sets in $\sset'$ are disjoint and of size at most $k$. Moreover, if event $\event$ does not happen, then
\[
\expect{|E(\sset')|}\ge 
\sum_{(u,v)\in E(\sset)}\Pr\Big[u,v\text{ belong to the same set in }\sset\Big]
\ge 
\sum_{(u,v)\in E(\sset)}\frac{1}{(4\log n)^2}
\ge \Omega\bigg(\frac{|E(\sset)|}{\log^2 n}\bigg).
\]
However, collection $\sset'$ may contain up to $(4n\log n/k)$ sets. We let $\sset''$ contain $n/k$ sets in $\sset'$ that contribute most edges in $E(\sset')$, so $|E(\sset'')|\ge \Omega(|E(\sset')|/\log n)$.
On the other hand, note that
\[\begin{split}
\expect{|E(\sset)|}= & \text{ }
\Pr[\overline{\event}]\cdot
\expect{ |E(\sset)| \text{ }\Big| \text{ } \overline{\event}}
+
\Pr[\event]\cdot
\expect{ |E(\sset)| \text{ }\Big| \text{ } \event}\\
\le & \text{ }
\Pr[\overline{\event}]\cdot
\expect{ |E(\sset)| \text{ }\Big| \text{ } \overline{\event}}
+
O\bigg(\frac{1}{n^3}\bigg)\cdot
n^2.
\end{split}
\]
Recall that $\expect{|E(\sset)|}\ge\Omega(\optcl(G,k)/(\alpha(n)\log^2 n))$,
so
$\expect{|E(\sset)| \mid \overline\event}\ge \Omega(\optcl(G,k)/(\alpha(n)\log^2 n))$. 
Therefore, 
\[\expect{|E(\sset'')|\mid \overline\event}\ge
\Omega\bigg(\frac{\expect{|E(\sset')|\mid \overline\event}}{\log n}\bigg)
\ge 
\Omega\bigg(\frac{\expect{|E(\sset)|\mid \overline\event}}{\log^3 n}\bigg)
\ge
\Omega\bigg(\frac{\optcl(G,k)}{\alpha(n)\log^5 n}\bigg).\] 
We can finally augment sets in $\sset''$ by vertices in $V$ such that eventually the sets in $\sset''$ partition $V$ and all but one set contains exactly $k$ vertices, and output $\sset''$. 
We repeat the whole algorithm $n^3$ times and output the best feasible solution among all runs.
Since $\alpha(n)=o(n)$, it is easy to show that, with probability $1-2^{-n}$, the final output is an $O(\alpha(n)\log^5 n)$-approximation of instance $\pcl(G,k)$.








\subsection{From bipartite graphs to general graphs}
\label{sec: bipartite to general}

In this subsection we show that, in order to obtain an approximation algorithm for \DkC or \WGP, it suffices to construct such an algorithm that works on bipartite graphs.


\begin{lemma}
\label{lem: bipartite_DkC}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. If there is an efficient $\alpha(n)$-approximation algorithm for \DkC on bipartite graphs, then there is an efficient $O(\alpha(n))$-approximation algorithm for \DkC.
\end{lemma}

\begin{lemma}
\label{lem: bipartite_WGP}
Let $\alpha: \mathbb{Z^+}\to \mathbb{Z^+}$ be an increasing function such that $\alpha(n)=o(n)$. If there is an efficient $\alpha(n)$-approximation algorithm for \WGP on bipartite graphs, then there is an efficient $O(\alpha(n))$-approximation algorithm for \WGP.
\end{lemma}

We only provide the proof of \Cref{lem: bipartite_DkC} here. The proof of \Cref{lem: bipartite_WGP} is very similar to the proof of \Cref{lem: bipartite_DkC}, and is deferred to \Cref{apd: Proof of bipartite_WGP}.

Let $\alg$ be an $\alpha(n)$-approximation algorithm for \DkC on bipartite graphs. We now construct an $O(\alpha(n))$-approximation algorithms for \DkC as follows. 
Let $\pcl(G,k)$ be the input instance where $G=(V,E)$. We first construct a bipartite graph $H=(V^1,V^2,E')$ as follows: $V^1=\set{v^1\mid v\in V}$, $V^2=\set{v^2\mid v\in V}$, and $E'=\set{(v^1,u^2), (v^2,u^1)\mid (v,u)\in E}$.
Consider now the instance $\pcl(H,2k)$. We apply the algorithm $\alg$ to it, and let $\sset'$ be the solution we get. Since $\alg$ is an $\alpha(n)$-approximation algorithm, $|E_H(\sset')|\ge \optcl(H,2k)/\alpha(n)$. 

On the one hand, we show that $\optcl(H,2k)\ge 2\cdot \optcl(G,k)$. Observe that, for any solution $\tset$ of instance $\pcl(G,k)$, we can construct a solution $\tset'$ to instance $\pcl(H,2k)$ as follows. For each set $T\in \tset$, we define $T'=\set{v^1,v^2\mid v\in T}$. We then let $\tset'=\set{T'\mid T\in \tset}$. It is easy to verify that, for each $T\in \tset$, $|T'|=2|T|$ and $|E_H(T')|=2|E_G(T)|$. Therefore, $\tset'$ is a valid solution to $\pcl(H,2k)$ and $|E(\tset')|\ge 2|E(\tset)|$, and so $\optcl(H,2k)\ge 2\cdot \optcl(G,k)$.

On the other hand, we can construct a solution $\tilde \sset$ to instance $\pcl(G,k)$ using the solution $\sset'$, such that $\expect{|E(\tilde\sset)|}\ge \Omega\big(\optcl(H, 2k)/\alpha(n)\big)$.

We first construct a collection $\sset$ of vertex subsets of $V$ that contains, for each set $S'\in \sset'$, a set $S\subseteq V$ constructed as follows.
For each vertex $v\in V$: 
\begin{itemize}
\item if both $v^1, v^2$ belong to the same set $S'\in \sset'$, then we add $v$ to $S$; 
\item if $v^1\in S'_1$ and $v^2\in S'_2$ (where $S'_1, S'_2$ are distinct sets in $\sset'$), then we add $v$ to $S_1$ (the set in $\sset$ corresponding to $S'_1$) with probability $1/2$ and add $v$ to $S_2$ (the set in $\sset$ corresponding to $S'_2$) with probability $1/2$.
\end{itemize}
It is easy to verify that every set $S\in \sset$ has size at most $2k$. Moreover, for each edge $(u^1,v^2)\in E(\sset')$, the probability that $(u,v)$ appears in $E(\sset)$ is at least $1/2$. Therefore,
\[
\expect{ |E(\sset)| }\ge 
\sum_{u,v\in V}\mathbf{1}{(u^1,v^2)\in E(\sset')\text{ or }(u^2,v^1)\in E(\sset')}\cdot \frac 1 2
\ge \frac{|E(\sset')|}{2}\cdot \frac 1 2=\frac{|E(\sset')|}{4}.
\]
For each set $S\in \sset$, if $|S|>k$, then we apply the algorithm from \Cref{lem: size reducing} to it and get a set $\tilde S\subseteq S$ with $|\tilde\sset|=k$ and $|E_G(\tilde S)|=\Omega(|E_G(S)|)$. We let set $\tilde\sset$ contains all sets $\tilde S$, and augment $\tilde\sset$ with all but one size-$k$ vertex sets in $G$ until $\tilde\sset$ is a valid solution to instance $\pcl(G,k)$. Therefore, we get that 
\[
\expect{ |E(\tilde\sset)| }\ge \Omega\bigg(\expect{|E(\sset)|}\bigg)\ge \Omega\bigg(\frac{|E(\sset')|}{4}\bigg)\ge \Omega\bigg(\frac{\optcl(H,2k)}{\alpha(n)}\bigg).
\]
Altogether, $\expect{ |E(\tilde\sset)|}=\Omega(\optcl(G,k)/\alpha(n))$.
Therefore, our algorithm returns an $O(\alpha(n))$-approximate solution to instance $\pcl(G,k)$.
















==> apd_WGP_to_DkS.tex <==
\section{Proofs Omitted from \Cref{sec: DkC and WGP to DkS}}


\subsection{Proof of \Cref{lem: sep to solve LP}}
\label{apd: Proof of sep to solve LP}


\newcommand{\sP}{{\sf P}}
\newcommand{\algo}{{\sf Alg}}
\newcommand{\fea}{{\sf Feasibility}}

We assume without loss of generality that the Linear Programs $\sP$ and $\sP'$ are given in the standard form, as follows.
%
\begin{eqnarray*}
	\mbox{$(\sP)$}	& &\\
	\max& \sum_{i=1}^m c_i\cdot x_i&\\
	\mbox{s.t.}&&\\
	&\sum_{i=1}^m A_{j,i}x_i\leq b_j &\forall 1\le j\le n\\
	&x_i\geq 0&\forall 1\le i\le m
\end{eqnarray*}
%
\begin{eqnarray*}
	\mbox{$(\sP')$}&&\\
	\min& \sum_{j=1}^n b_j\cdot y_j&\\
	\mbox{s.t.}&&\\
	&\sum_{j=1}^n A_{j,i}y_j\geq c_i &\forall 1\le i\le m\\
	&y_j\geq 0&\forall 1\le j\le n
\end{eqnarray*}

For a solution $x$ to $\sP$, we denote its value $\val(\sP,x)=\sum_{i=1}^mc_ix_i$, and we define $\val(\sP',y)$ similarly for any solution $y$ to $\sP'$. 
%
Note that $\sP$ has $m$ variables and $\sP'$ has $n$ variables. We denote by $L=L(\sf P)$.
We denote by $\opt(\sP)$ and $\opt(\sP')$ the values of the optimal solutions to $\sP$ and $\sP'$, respectively. From the Strong Duality Theorem, $\opt(\sP)=\opt(\sP')$.


By repeating the separation oracle for $\sP'$ $4n$ times, we obtain a $\beta(n)$-approximate separation oracle for $\sf P'$, that we denote by $\alg$, which errs with probability at most $2^{-4n}$.

\paragraph{The Algorithm.}
For a real value $v$, we denote by $\sP'(v)$ the feasibility LP obtained from $\sP'$ by replacing its objective function with the constraint $\sum_{j=1}^n b_j\cdot y_j=v$. We then consider a randomized algorithm, that we denote by $\algo'(\sP',v)$, that applies the Ellipsoid algorithm, together with the separation oracle $\aset$, to $\sP'(v)$. 
@@@ Recall thatTherefore, $\fea(\sP',v)$ either reports that $\sP'(v)$ is infeasible, or returns a vector $y\in \mathbb{R}^n$ such that $\sum_{1\le j\le n} b_j\cdot y_j=v$ and $\sum_{1\le j\le n} a_{ji}y_j\geq c_i/\beta(n)$ for all $1\le i\le m$.

Consider the following algorithm $\algo$ for computing a solution to $\sP'$ using the Ellipsoid algorithm and the approximate separation oracle $\alg$:
%For each real number $v$, we denote by $\sP'(v)$ the feasibility LP obtained from $\sP'$ by replacing its objective function with a constraint $\sum_{1\le j\le n} b_j\cdot y_j=v'$. We say that $\sP'(v)$ is \emph{approximately feasible} iff there is a solution $y$, such that $\sum_{1\le j\le n} b_j\cdot y_j=v'$ and $\sum_{1\le j\le n} a_{ji}y_j\leq c_i\cdot\beta(n)$ for all $1\le i\le m$.
For each real number $v$, 
%
We use binary search to find the maximum value $V$, such that the process $\fea(\sP',V)$ returns a vector, and let $y^*$ be the solution returned by the process $\fea(\sP',V)$.

Let $J$ be the set of all constraints that are ever returned by the separation oracle $\alg$ as a violating constraint. We define $\hat \sP'$ as the LP obtained from $\sP'$ by only keeping the constraints in $J$. Note that each constraint in $J$ corresponds to a variable in $\sP$, and we define $\hat \sP$ as the LP obtained from $\sP$ by only keeping the variables that correspond to some constraint in $J$ (e.g., if we only keep variable $x_1,x_3$ from the constraint $x_1+2x_2+3x_3\le 4$, then the constraint we get is $x_1+3x_3\le 4$). 
%Since the Ellipsoid algorithm runs in polynomial time, the algorithm $\alg$ also runs in polynomial time, and therefore the number of constraints in $J$ is polynomial in $n$.

We then solve $\hat \sP$. Let $\hat x$ be the solution we get. We then construct a solution $x^*$ to $\sP$ as follows. For each variable $x_i$ whose corresponding dual constraint in $\sP'$ lies in $J$, we set $x^*_i=\hat x_i$; for each variable $x_i$ whose corresponding dual constraint in $\sP'$ does not lie in $J$, we set $x^*_i=0$.
Finally, we return $x^*$ as a solution to $\sP$.
This completes the description of the algorithm $\algo$.

\paragraph{Analysis of running time.}
Recall that we denote by $L(\sf P)$ the largest number of bits needed to represent any coefficient in $\sf P$. Since LPs $\sf P$ and $\sf P'$ has same coefficients, $L(\sf P)= L(\sf P')$. 
Since we perform binary search to find the maximum value $V$ such that $\fea(\sP',v)$ returns a vector (instead of reporting infeasibility), the number of process $\fea(\sP',\cdot)$ that we perform is at most $O(L(\sf P))$, as the optimal value of $\sf P'$ contains at most $O(L(\sf P))$ digits (since we can set all $y_j=\frac{\max\set{c_i\mid 1\le i\le m}}{\min\set{a_{i,j}\ne 0\mid 1\le i\le m,1\le j\le n}}$ and achieve an $O( L(\sf P))$-digit objective value of the LP $\sf P'$). Since every implementation of the process takes time $\poly(n\cdot L(\sf P))$ (as the running time of the separation oracle is polynomial in its input length, the length of $n$ real numbers $y_1,\ldots, y_n$, which is at most $n\cdot L(\sf P)$ since each $y_i$ has length at most $L(\sf P)$), the running time caused by the implementation of the separation oracle $\alg$ is $\poly(n\cdot L(\sf P))$.

On the other hand, since the number of constraints in $J$ is polynomial in $n\cdot L(\sP)$ (as the running time of the algorithm $\algo$ is $\poly(n\cdot L(\sP))$), and recall that $(\sP)$ contains $n$ constraints, we get that the LP $\hat \sP$ has $\poly(n\cdot L(\sP))$ constraints and $n$ variables. Therefore, solving $\hat \sP$ takes $\poly(n\cdot L(\sP))$ time.


\paragraph{Proof of Correctness.}
We say that an implementation of $\alg$ is \emph{unsuccessful}, iff either it reports that all constraints are approximately satisfied but the report is incorrect; or it returns a constraint that is not violated. Otherwise we say it is successful. Since $\alg$ is a $\beta(n)$-approximate separation oracle with unsuccessful probability $2^{-\Omega(n\cdot L(\sf P))}$, we get that the probability that an implementation of $\alg$ is unsuccessful is $2^{-\Omega(n\cdot L(\sf P))}$.
Since the running time of $\algo$ is $\poly(n\cdot L(\sf P))$, it implements the separation oracle $\alg$ at most $\poly(n\cdot L(\sf P))$ times. Therefore, the the probability that any of these implementation of $\alg$ is unsuccessful is at most $2^{-\Omega(n\cdot L(\mathsf{P}))}\cdot \poly(n\cdot L(\mathsf{P}))=o(1)$.

We now show that, if all implementations of the separation oracle $\alg$ in $\algo$ are successful, then the solution $x^*$ returned by the algorithm $\algo$ is a $\beta(n)$-approximate solution to $\sP$. Note that, if all implementations of the separation oracle $\alg$ are successful, then all implementations of the process $\fea(\sP', v)$ report correctly.


We prove the following observations.

\begin{observation}
\label{obs: 1}
If all implementations of the separation oracle $\alg$ are successful, then $V\le \textnormal{OPT}(\sP)\le V\cdot \beta(n)$. 
\end{observation}
\begin{proof}
We define a vector $y'\in \mathbb{R}^n$ as follows: $y'_j=\beta(n)\cdot y^*_j$ for all $1\le j\le m$.
Since $\sum_{1\le j\le n} a_{ji}y^*_j\geq c_i/\beta(n)$ for all $1\le i\le m$, we get that $\sum_{1\le j\le n} a_{ji}y'_j\geq c_i$ for all $1\le i\le m$, namely $y'$ is a feasible solution to $\sP'$, and so \[\textnormal{OPT}(\sP')\le \val(\sP',y)=\sum_{1\le j\le n}b_jy'_j\le \sum_{1\le j\le n}b_jy^*_j\cdot \beta(n)= V\cdot \beta(n).\] 
On the other hand, since for any $v<V$, the process $\fea(\sP',v)$ reports that $\sP'(v)$ is infeasible, we get that $\opt(\sP')\ge V$. The observation now follows from the fact that $\opt(\sP)=\opt(\sP')$.
\end{proof}



%Let $J$ be the set of all constraints that are ever returned by the separation oracle $\alg$ as a violating constraint. We define $\hat \sP'$ as the LP obtained from $\sP'$ by only keeping the constraints in $J$. Note that each constraint in $J$ corresponds to a variable in $\sP$, and we define $\hat \sP$ as the LP obtained from $\sP$ by only keeping the variables that correspond to some constraint in $J$ (e.g., if we only keep variable $x_1,x_3$ from the constraint $x_1+2x_2+3x_3\le 4$, then the constraint we get is $x_1+3x_3\le 4$). Since the Ellipsoid algorithm runs in polynomial time, the algorithm $\alg$ also runs in polynomial time, and therefore the number of constraints in $J$ is polynomial in $n$. We prove the following observation.

\begin{observation}
\label{obs: 2}
If all implementations of the separation oracle $\alg$ are successful, then $\textnormal{OPT}(\hat \sP)=\textnormal{OPT}(\sP)$.
\end{observation}
\begin{proof}
It is easy to verify that $\hat \sP'$ is the dual of $\hat \sP$. Therefore, from the Strong Duality, $\textnormal{OPT}(\sP_J)=\textnormal{OPT}(\hat \sP')$. Also note that, if we apply the algorithm $\algo$ to $\hat \sP'$, then the run of the Ellipsoid algorithm is identical to the run when it is applied to $\sP'$, and so we get the same output $V$ and $y^*$.
Altogether, $\textnormal{OPT}(\hat \sP)=\textnormal{OPT}(\hat \sP')=\textnormal{OPT}(\sP')$. Since $\textnormal{OPT}(\sP)=\textnormal{OPT}(\sP')$, we get that $\textnormal{OPT}(\hat \sP)=\textnormal{OPT}(\sP)$.
\end{proof}

%Since the number of constraints in $J$ is polynomial in $n\cdot L(\sP)$ (as the running time of the algorithm $\algo$ is $\poly(n\cdot L(\sP))$), and recall that $(\sP)$ contains $n$ constraints, we get that the LP $\hat \sP$ has $n$ constraints and $n$ variables. We then solve $\hat \sP$, which takes polynomial time (in $n$). Let $\hat x$ be the solution we get.
From \Cref{obs: 1} and \ref{obs: 2}, $V\le \val(\hat \sP,\hat x)\le \beta(n)\cdot V$. From the construction of solution $x^*$, it is easy to verify that $\val(\sP, x^*)=\val(\hat \sP,\hat x)$. Therefore, $V\le \val(\sP, x^*)\le \beta(n)\cdot V$. From \Cref{obs: 1}, we get that $x^*$ is an $\beta(n)$-approximate solution to $\sP$.




\subsection{Reduction from \WGP to \DkS}
\label{apd: WGP to DkS}

In this subsection we provide the proof of the second half of \Cref{thm: alg_DkS gives alg_DkC} by showing a reduction from \WGP to \DkS. The reduction is quite similar to the reduction shown in \Cref{sec: DkC and WGP to DkS}. 

Let $\pwgp(G,r,h)$ be the input instance of \WGP.
We denote $V=V(G)$ and $N=|V|$.
We assume that $\log_2 n$ is an integer. We denote by $\rset$ the collection of all subsets $S$ of $V$ with $|E_G(S)|\le h$. We consider the following LP, whose variables are $\set{x_S}_{S\in \rset}$.
%
\begin{eqnarray*}
	\mbox{(LP-1)}	&\text{maximize } \sum_{S\in \rset} x_S\cdot |E_G(S)|\\
	\mbox{s.t.}&&\\
	&\sum_{S: v\in S} x_S\leq 1 &\forall v\in V\\
	&\sum_{S\in \rset}x_S \leq r\\
	&x_S\geq 0&\forall S\in \rset
\end{eqnarray*}
%
We show in the following claim that $\opt(\textnormal{LP-1})\ge \Omega(\optwgp(G,r,h))$.
\begin{claim}
$\textnormal{OPT}(\textnormal{LP-1})\ge \optwgp(G,r,h)/3$.
\end{claim}
\begin{proof}
We prove the following observation.

\begin{observation}
\label{obs: shrink set}
There is an efficient algorithm, that, given any graph $G$, any integer $\hat h$ and any set $S\subseteq V(G)$ such that $|E(S)|\ge \hat h$, computes a subset $S'\subseteq S$, such that $\hat h/3\le |E(S')|\le \hat h$.
\end{observation}
\begin{proof}
The algorithm is similar to the algorithm in the proof of \Cref{lem: size reducing}. Observe that, if $H$ is an $n$-vertex (where $n\ge 3$) graph, and $v$ is a lowest-degree vertex of $H$, then the degree of $v$ in $H$ is at most $2|E(H)|/n$. Therefore, if vertex $v$ is removed from $H$, then $|E(H)|$ decreases by at most a factor $(1-2/n)$. 

Consider now the graph $G'=G[S]$ and denote $|S|=k$. If we iteratively remove the lowest-degree vertex from $G'$, until $G'$ becomes an empty graph, and let $G_k=G',G_{k-1},\ldots,G_0=\empty$ be the graphs we get, then $|E(G_k)|\ge \hat h$, $|E(G_2)|\le 3$, and for each $3\le i\le k$, \[|E(G_i)|\cdot \bigg(1-\frac{2}{i}\bigg)\le |E(G_{i-1})|\le |E(G_i)|.\]
If $\hat h\le 3$, then clearly the observation holds (since we can set $S'$ to be any pair of adjacent vertices in $S$). If $\hat h\ge 4$, then there must be some index $3\le i\le k+1$, such that $|E(G_{i-1})|\le \hat h < |E(G_i)|$. We find such a index $i$ and simply set $S'=V(G_{i-1})$. Note that $|E(S')|=|E(G_{i-1})|\le \hat h$, and 
\[|E(S')|=|E(G_{i-1})|\ge|E(G_i)|\cdot \bigg(1-\frac{2}{i}\bigg)\ge \hat h\cdot\bigg(1-\frac{2}{3}\bigg)=\frac{\hat h}{3}.\]
This completes the proof of the observation.
\end{proof}

Let $\hset=\set{H_1,\ldots,H_r}$ be any solution to instance $\pwgp(G,r,h)$. For each $1\le i\le r$, we denote $S_i=V(H_i)$, so sets $S_1,\ldots,S_r$ are mutually disjoint and $|E_G(S_i)|\ge |E(H_i)|$ for all $i$. If $|E_G(S_i)|\le h$, then we let $S'_i=S_i$. If $|E_G(S_i)|> h$, then we let $S'_i$ be the set obtained by applying \Cref{obs: shrink set} to graph $G$, integer $h$ and set $S_i$, so $h/3\le |E(S'_i)|\le h$ and so $|E(S'_i)|\ge |E(H_i)|/3$. We now define a solution $x'$ to (LP-1) as follows, for each $i$, we set $x'_{S_i}=1$; and for all other sets $S\in \rset$, we set $x'_S=0$. It is easy to verify that $x'$ is a feasible solution to (LP-1). On the other hand, since $|E(S'_i)|\ge |E(H_i)|/3$ for each $i$, we get that 
\[\sum_{S\in \rset}x'_S\cdot |E(S)|=\sum_{1\le i\le r}x'_{S_i}\cdot |E(S_i)|\ge \sum_{1\le i\le r}x'_{S_i}\cdot |E(H_i)|/3.\]
It follows that $\opt(\textnormal{LP-1})\ge \optwgp(G,r,h)/3$.
\end{proof}


We consider the following LP whose variables are $z$ and $\set{y_v}_{v\in V}$, that is the dual of (LP-1).
%
\begin{eqnarray*}
	\mbox{(LP-2)}	&\text{minimize } r\cdot z+\sum_{v\in V} y_v\\
	\mbox{s.t.}&&\\
	& z+\sum_{v\in S} y_v\geq |E_G(S)| &\forall S\in \rset\\
	&z\ge 0\\
	&y_v\geq 0&\forall v\in V
\end{eqnarray*}
%






The remainder of this subsection is divided into two parts. In the first part, we construct an efficient $O(\alpha(N^2)\log^2N)$-approximate separation oracle for (LP-2), using the approximate algorithm for \DkS. From \Cref{lem: sep to solve LP}, we can then use it to efficiently compute an $O(\alpha(N^2)\log^2N)$-approximate solution to (LP-1). In the second part, we compute an $O(\alpha(N^2)\log^5N)$-approximate solution to instance $\pwgp(G,r,h)$ using the approximate solution to (LP-1).

Since we assume that there exists an efficient $\alpha(n)$-approximation algorithm for \DkS, where $n$ is the number of vertices in the input graph, from \Cref{lem: DkS and Dk1k2S}, there exists an efficient $c_0\cdot \alpha(N^2)$-approximation algorithm for \BDkS, where $N$ is the number of vertices in the input graph and $c_0$ is some constant. We denote this algorithm by $\algdbs$.


We now describe the construction of an approximate separation oracle for (LP-2).

\subsubsection*{An approximate separation oracle for (LP-2)}

We define $\beta(N)=4000\cdot c_0\cdot \alpha(N^2)\log^5N$.

Let $(z,\set{y_v}_{v\in V})$ be the input real numbers. Recall that $|V|=N$. We will construct an efficient algorithm, that, with probability $1-2^{-\Omega(N)}$, either correctly reports that $z+\sum_{v\in V} y_v\geq |E_G(S)|/\beta(N)$ holds for all $S\in \rset$, or find a set $S\subseteq V, S\in \rset$ such that $z+\sum_{v\in V} y_v< |E_G(S)|$.


We define a process $\algsep$ that serves as a building block of the algorithm. The process $\algsep$ either returns a violating constraint, or returns {\sf Fail}.

We first pick a random partition of $V$ into two sets $V=A\cup B$. That is, for every vertex of $V$, with probability $1/2$ it lies in $A$, and with probability $1/2$ it lies in $B$. We then define the bipartite graph $G'=(A,B,E_G(A,B))$.
%
We denote $L=-4\log N$ and $L'=2\log N$. For each integer $L\le t\le L'$, we define $A_t=\set{v\in A\mid 2^t\le y_v <2^{t+1}}$ and $B_t=\set{v\in B\mid 2^t\le y_v <2^{t+1}}$, and we denote $A_{L-1}=A\setminus \big(\bigcup_{L\le t\le L'}A_t\big)$ and $B_{L-1}=B\setminus \big(\bigcup_{L\le t\le L'}B_t\big)$, so for all vertices $v\in A_{L-1}\cup B_{L-1}$, we have $y_v<1/N^4$.

%\tnote{getting rid of small coordinates in the construction of separation oracle}

We say that a pair $(k_1,k_2)$ of integers are \emph{eligible}, iff $k_1,k_2\ge 0$ and $k_1+k_2\le N$. Then:
\begin{itemize}
	\item For each eligible pair $(k_1,k_2)$, and for each pair $L-1\le i,j\le L'$, we apply the approximation algorithm for \BDkS to instance $\pbdks(G'[A_i\cup B_j],k_1,k_2)$, and let $S^{k_1,k_2}_{i,j}$ be the solution we get, so $|E(S^{k_1,k_2}_{i,j})|\ge \optbdks(G'[A_i\cup B_j],k_1,k_2)/(c_0\cdot \alpha(N^2))$. We then check if the inequality 
	\[z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v\geq \min\bigg\{|E_{G}(S^{k_1,k_2}_{i,j})|,\frac{h}{4}\bigg\}\] 
	holds. If not, then 
	\begin{itemize}
	\item if $|E_{G}(S^{k_1,k_2}_{i,j})|\le h$, then the process returns $z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v\geq |E_{G}(S^{k_1,k_2}_{i,j})|$ as violating constraint (and clearly the report is correct);
	\item if $|E_{G}(S^{k_1,k_2}_{i,j})|> h$, then we apply the algorithm from \Cref{obs: shrink set} to graph $G$, integer $h$ and set $S^{k_1,k_2}_{i,j}$, and let $\hat S^{k_1,k_2}_{i,j}$ be the set we get;
	the process returns the following constraint as violating constraint: \[z+\sum_{v\in \hat S^{k_1,k_2}_{i,j}} y_v\geq |E_{G}(\hat S^{k_1,k_2}_{i,j})|.\]
	From \Cref{obs: shrink set}, $h/3\le |E(\hat S^{k_1,k_2}_{i,j})|\le h$, so $z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v< h/4< |E_{G}(\hat S^{k_1,k_2}_{i,j})|$, and the report is correct.
	\end{itemize}
	\item For each eligible pair $(k_1,k_2)$, and for each $L\le j\le L'$, we apply the approximation algorithm for \BDkS to instance $\pbdks(G'[A_i\cup B_j],k_1,k_2)$, and let $S^{k_1,k_2}_{i,j}$ be the solution we get, so $|E(S^{k_1,k_2}_{i,j})|\ge \optbdks(G'[A_i\cup B_j],k_1,k_2)/(c_0\cdot \alpha(N^2))$. We check if the inequality 
	$$z+\sum_{v\in (S^{k_1,k_2}_{L-1,j}\cap B)} y_v\ge \min\bigg\{|E_{G}(S^{k_1,k_2}_{L-1,j})|,\frac{h}{4}\bigg\}$$
	holds.
	If not, then 
	\begin{itemize}
	\item if $|E_{G}(S^{k_1,k_2}_{L-1,j})|\le h$, then the process returns $z+\sum_{v\in S^{k_1,k_2}_{L-1,j}} y_v\geq |E_{G}(S^{k_1,k_2}_{L-1,j})|$ as violating constraint (and clearly the report is correct);
	\item if $|E_{G}(S^{k_1,k_2}_{L-1,j})|> h$, then we apply the algorithm from \Cref{obs: shrink set} to graph $G$, integer $h$ and set $S^{k_1,k_2}_{L-1,j}$, and let $\hat S^{k_1,k_2}_{L-1,j}$ be the set we get;
	the process returns the following constraint as violating constraint: \[z+\sum_{v\in \hat S^{k_1,k_2}_{L-1,j}} y_v\geq |E_{G}(\hat S^{k_1,k_2}_{L-1,j})|.\]
	From \Cref{obs: shrink set}, $h/3\le |E(\hat S^{k_1,k_2}_{L-1,j})|\le h$, so $z+\sum_{v\in S^{k_1,k_2}_{L-1,j}\cap B} y_v< h/4< |E_{G}(\hat S^{k_1,k_2}_{L-1,j})|\cdot (3/4)$. Moreover, since $y_v<1/N^4$ for all $v\in A_{L-1}\cup B_{L-1}$, $\sum_{v\in S^{k_1,k_2}_{i,L-1}\cap A} y_v< N\cdot(1/N^4)<1/N^3< |E_{G}(\hat S^{k_1,k_2}_{L-1,j})|/4$. Combined together, we get that the report is correct.
\end{itemize}
\item For each eligible pair $(k_1,k_2)$, and for each $L\le i\le L'$,  we apply the approximation algorithm for \BDkS to instance $\pbdks(G'[A_i\cup B_j],k_1,k_2)$, and let $S^{k_1,k_2}_{i,j}$ be the solution we get, so $|E(S^{k_1,k_2}_{i,j})|\ge \optbdks(G'[A_i\cup B_j],k_1,k_2)/(c_0\cdot \alpha(N^2))$. We check if the inequality 
$$z+\sum_{v\in (S^{k_1,k_2}_{i,L-1}\cap A)} y_v\ge \min\bigg\{\frac{|E_{G}(S^{k_1,k_2}_{i,L-1})|}{2},\frac{h}{4}\bigg\}$$
holds.
If not, then 
\begin{itemize}
	\item if $|E_{G}(S^{k_1,k_2}_{i,L-1})|\le h$, then the process returns $z+\sum_{v\in S^{k_1,k_2}_{i,L-1}} y_v\geq |E_{G}(S^{k_1,k_2}_{i,L-1})|$ as violating constraint (and clearly the report is correct);
	\item if $|E_{G}(S^{k_1,k_2}_{i,L-1})|> h$, then we apply the algorithm from \Cref{obs: shrink set} to graph $G$, integer $h$ and set $S^{k_1,k_2}_{i,L-1}$, and let $\hat S^{k_1,k_2}_{i,L-1}$ be the set we get;
	the process returns the following constraint as violating constraint: \[z+\sum_{v\in \hat S^{k_1,k_2}_{i,L-1}} y_v\geq |E_{G}(\hat S^{k_1,k_2}_{i,L-1})|.\]
	From \Cref{obs: shrink set}, $h/3\le |E(\hat S^{k_1,k_2}_{i,L-1})|\le h$, so $z+\sum_{v\in S^{k_1,k_2}_{i,L-1}\cap A} y_v< h/4< |E_{G}(\hat S^{k_1,k_2}_{i,L-1})|\cdot (3/4)$. Moreover, since $y_v<1/N^4$ for all $v\in A_{L-1}\cup B_{L-1}$, $\sum_{v\in S^{k_1,k_2}_{i,L-1}\cap B} y_v< N\cdot(1/N^4)<1/N^3< |E_{G}(\hat S^{k_1,k_2}_{i,L-1})|/4$. Combined together, we get that the report is correct.
\end{itemize}
	\item Lastly, for each eligible pair $(k_1,k_2)$, we check if $z\ge \min\set{|E_{G}(S^{k_1,k_2}_{L-1,L-1})|/2,h/4}$ holds. If not, then 
	\begin{itemize}
		\item if $|E_{G}(S^{k_1,k_2}_{L-1,L-1})|\le h$, then the process returns $z+\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v\geq |E_{G}(S^{k_1,k_2}_{L-1,L-1})|$ as violating constraint. To see why the report is correct, note that $|E_{G}(S^{k_1,k_2}_{L-1,L-1})|\ge 1$, and since $y_v\le 1/N^4$ for all $v\in S^{k_1,k_2}_{L-1,L-1}$, we get that $\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v<|E_{G}(S^{k_1,k_2}_{L-1,L-1})|/2$. Therefore,
		$$z+\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v< \min\bigg\{\frac{|E_{G}(S^{k_1,k_2}_{L-1,L-1})|}{2},\frac{h}{4}\bigg\}+\frac{|E_{G}(S^{k_1,k_2}_{L-1,L-1})|}{2}\le |E_{G}(S^{k_1,k_2}_{L-1,L-1})|,$$
		and the report is correct.
		\item if $|E_{G}(S^{k_1,k_2}_{L-1,L-1})|> h$, then we apply the algorithm from \Cref{obs: shrink set} to graph $G$, integer $h$ and set $S^{k_1,k_2}_{L-1,L-1}$, and let $\hat S^{k_1,k_2}_{L-1,L-1}$ be the set we get;
		the process returns the following constraint as violating constraint: \[z+\sum_{v\in \hat S^{k_1,k_2}_{L-1,L-1}} y_v\geq |E_{G}(\hat S^{k_1,k_2}_{L-1,L-1})|.\]
		From \Cref{obs: shrink set}, $h/3\le |E(\hat S^{k_1,k_2}_{L-1,L-1})|\le h$. Since $\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v<|E_{G}(S^{k_1,k_2}_{L-1,L-1})|/2$, so $z+\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v< h/4+1/N^4< |E_{G}(\hat S^{k_1,k_2}_{L-1,L-1})|$, and the report is correct.
	\end{itemize}
\end{itemize}
If the process did not find a violating constraint in the above steps, then the process returns {\sf Fail}. This completes the description of the process $\algsep$.

The algorithm simply repeat the process  $\algsep$ $N^2$ times. If any run of the process $\algsep$ returns a violating constraint, then the algorithm returns the same constraint as a violating constraint. If all runs of the process $\algsep$ returns {\sf Fail}, then the algorithm reports that, for all sets $S\subseteq V$ with $S\in \rset$, $z+\sum_{v\in V} y_v\geq |E_G(S)|/\beta(N)$ holds. This completes the description of the algorithm.


It remains to show that the above algorithm is indeed a $\beta(N)$-approximate separation oracle. 

\paragraph{Bad Event $\event$.}
For every set $S\in \rset$, we define $\event_S$ to be the bad event that, in every run of the process, the graph $G'$ constructed at the beginning contains less than $(1/10)$-fraction of the edges in $E_G(S)$, i.e., $|E_{G'}(S)|\le |E_G(S)|/10$. Since graph $G'$ is determined by the random partition $(A,B)$ of $V$, $\expect[]{|E_{G'}(S)}=|E_G(S)|/2$. Since $|E_{G'}(S)|\le |E_G(S)|$ always holds, we get that with probability at least $1/3$, $|E_{G'}(S)|\ge |E_G(S)|/10$. Therefore, $\Pr[\event_S]\le (2/3)^{N^2}$. We then define $\event$ as the event that event $\event_S$ happens for some set $S\in \rset$. From the Union Bound on all sets in $\rset$, $\Pr[\event]\le (2/3)^{N^2}\cdot N^N\le 2^{-\Omega(N)}$.

We now show that, if $\event$ does not happen, then the algorithm reports correctly.



%
First, if the process returns a violated constraint through the process of processing a pair $(i,j)$ of indices, then from the above discussion, the returned constraint is indeed a violating constraint.
%$z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v\geq |E_{G}(S^{k_1,k_2}_{i,j})|$.
\iffalse
Then:
\begin{itemize}
	\item if $L\le i,j\le L'$, then
	 according to the process, we have confirmed that the constraint is indeed a violating constraint;
	\item if $i=L-1$ and $j\ne L-1$, then we have checked that $z+\sum_{v\in (S^{k_1,k_2}_{L-1,j}\cap B)} y_v< |E_{G}(S^{k_1,k_2}_{L-1,j})|/2$, so $|E_{G}(S^{k_1,k_2}_{L-1,j})|>1$, and since $\sum_{v\in (S^{k_1,k_2}_{L-1,j}\cap A)} y_v<(1/N^4)\cdot N=1/N^3$, $z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v< |E_{G}(S^{k_1,k_2}_{i,j})|$, so the returned constraint is indeed a violating constraint;
	\item if $j=L-1$ and $i\ne L-1$, then we have checked that $z+\sum_{v\in (S^{k_1,k_2}_{i,L-1}\cap A)} y_v< |E_{G}(S^{k_1,k_2}_{i,L-1})|/2$, so $|E_{G}(S^{k_1,k_2}_{i,L-1})|>1$, and since $\sum_{v\in (S^{k_1,k_2}_{i,L-1}\cap N)} y_v<(1/N^4)\cdot N=1/N^3$, $z+\sum_{v\in S^{k_1,k_2}_{i,j}} y_v< |E_{G}(S^{k_1,k_2}_{i,j})|$, so the returned constraint is indeed a violating constraint;
	\item if $i=j= L-1$, then we have checked that $z< |E_{G}(S^{k_1,k_2}_{L-1,L-1})|/2$, so $|E_{G}(S^{k_1,k_2}_{i,L-1})|>1$, and since $\sum_{v\in (S^{k_1,k_2}_{L-1,L-1}\cap N)} y_v<(1/N^4)\cdot N=1/N^3$, $z+\sum_{v\in S^{k_1,k_2}_{L-1,L-1}} y_v< |E_{G}(S^{k_1,k_2}_{L-1,L-1})|$, so the returned constraint is indeed a violating constraint;
\end{itemize}
%Therefore, the algorithm reports correctly in this case. 
\fi


Consider now the case where the algorithm did not find a violating constraint. This means all $N^2$ runs of the process $\algsep$ failed to find a violating constraint. 
%
Let $S$ be any set in $\rset$, so $|E_G(S)|\le h$. We now show that the constraint $z+\sum_{v\in S} y_v\geq |E_{G}(S)|$ is satisfied.
%Assume for contradiction that the constraint is not satisfied.
%
For each pair $L-1\le i,j\le L'$, we denote $p_i=|S\cap A_{i}|$ and $q_j=|S\cap B_{j}|$. Since $|S|\le k$, $|S\cap A_{i}|+|S\cap B_{j}|\le k$, so $(p_i,q_j)$ is an eligible pair. Since event $\event_S$ does not happen, there exists a run of the process $\algsep$, such that $|E_{G'}(S)|\ge |E_G(S)|/10$. From now on we consider this run of the process $\algsep$.
% and show that this run must return a violating constraint instead of returning {\sf Fail}, leading to a contradiction.

For every pair $L\le i,j\le L'$, recall that we have applied the approximation algorithm for \BDkS to instance $\pbdks(G'[A_i\cup B_j],p_i,q_j)$, found a solution $S^{p_i,q_j}_{i,j}$, and certified that
$z+\sum_{v\in S^{p_i,q_j}_{i,j}} y_v\geq \min\set{|E_G(S^{p_i,q_j}_{i,j})|,h/4}$. 
Since $|E_G(S)|\le h$, $z+\sum_{v\in S^{p_i,q_j}_{i,j}} y_v\geq |E_G(S^{p_i,q_j}_{i,j})|/4$. 
Since $G'$ is a subgraph of $G$, $|E_G(S^{p_i,q_j}_{i,j})|\ge |E_{G'}(S^{p_i,q_j}_{i,j})|$, and so
\[z+\sum_{v\in S^{p_i,q_j}_{i,j}} y_v
\geq \frac{|E_{G}(S^{p_i,q_j}_{i,j})|}{4}
\geq \frac{|E_{G'}(S^{p_i,q_j}_{i,j})|}{4}\ge \frac{\optdks(G'[A_i\cup B_j],p_i,q_j)}{4c_0\cdot \alpha(N^2)}\ge \frac{|E_{G'}(S\cap A_i, S\cap B_j)|}{4c_0\cdot \alpha(N^2)}.\]
Note that $|S^{p_i,q_j}_{i,j}\cap A_i|=p_i=|S\cap A_i|$, $|S^{p_i,q_j}_{i,j}\cap B_j|=q_i=|S\cap B_j|$. Also note that the $y_v$ values for all vertices in $A_i$ are within factor $2$ from each other, and so are the $y_v$ values for all vertices in $B_j$. It follows that
\[\sum_{v\in (S\cap A_i)}y_v\ge \frac{1}{2}\cdot\bigg(\sum_{v\in S^{p_i,q_j}_{i,j}\cap A_i} y_v\bigg); \text{ and } \sum_{v\in (S\cap B_j)}y_v\ge \frac{1}{2}\cdot\bigg(\sum_{v\in S^{p_i,q_j}_{i,j}\cap B_j} y_v\bigg),\]
and so 
\[ z+\sum_{v\in S\cap (A_i\cup B_j)} y_v \ge \frac{|E_{G'}(S\cap A_i, S\cap B_j)|}{8c_0\cdot \alpha(N^2)}.\]
%

\iffalse
Therefore, summing over all pairs $L\le i,j\le L'$, we get that
\begin{equation}
\label{eq1}
30z\log^2 N+\sum_{v\in S'} y_v\geq  \sum_{L\le i,j\le L'}\frac{|E(S\cap A_i, S\cap B_j)|}{2\alpha(N)}\ge \frac{|E(S')|}{2\alpha(N)}.
\end{equation}
%
\fi


For every $L\le j\le L'$, recall that we have certified that $z+\sum_{v\in (S^{k_1,k_2}_{L-1,j}\cap B)} y_v\ge \min\set{|E_{G}(S^{k_1,k_2}_{L-1,j})|/2,h/4}$. From similar arguments, we can show that
\[ z+\sum_{v\in S\cap (A_{L-1}\cup B_j)} y_v \ge \frac{|E_{G'}(S\cap A_{L-1}, S\cap B_j)|}{8c_0\cdot \alpha(N^2)}.\]
Similarly, for every $L\le i\le L'$, we can show that
\[ z+\sum_{v\in S\cap (A_{i}\cup B_{L-1})} y_v \ge \frac{|E_{G'}(S\cap A_{i}, S\cap B_{L-1})|}{8c_0\cdot \alpha(N^2)}.\]
Lastly, we can show that
\[ z\ge \frac{|E_{G'}(S\cap A_{L-1}, S\cap B_{L-1})|}{8c_0\cdot \alpha(N^2)}.\]

Summing over the above four inequalities, we get that
\[(7\log N)^2\cdot z+\sum_{v\in S} y_v\geq   \frac{|E_{G'}(S)|}{8c_0\cdot \alpha(N^2)}.\]
Therefore, $z+\sum_{v\in S} y_v\geq  |E_{G'}(S)|/(400c_0\cdot \alpha(N^2)\cdot \log^2 N)$. Since in this run $|E_{G'}(S)|\ge |E_G(S)|/10$ holds, $z+\sum_{v\in S} y_v\geq  |E_{G}(S)|/(4000c_0\cdot \alpha(N^2)\cdot \log^2 N)$, and the report of the algorithm is correct. 


\subsubsection*{Computing a solution to instance $\pwgp(G,r,h)$}


Recall that we have computed a feasible solution $x^*$ to (LP-1) using the algorithm in \Cref{lem: sep to solve LP} and the approximate separation oracle constructed in the previous subsection, such that
\[\sum_{|E(S)|\le h}x^*_S\cdot |E(S)|\ge \Omega\bigg(\frac{\opt(\textnormal{LP-1})}{\alpha(N^2)\log^2 N}\bigg)\ge 
\Omega\bigg(\frac{\optwgp(G,r,h)}{\alpha(N^2)\log^2 N}\bigg).\]
We then let $\sset$ be the collection that contains each $S$ such that $S\in \rset$, set $S$ independently with probability $x^*_S$, so $\expect{|E(\sset)|}=\sum_{|S|\le k}x^*_S\cdot |E(S)|\ge\Omega(\optcl(G,k)/(\alpha(N^2)\log^2 N))$.
%
We use the following observation, whose proof is identical to \Cref{obs: bad event}, and is omitted here.
\begin{observation}
\label{obs: bad event apd}
With probability $1-O(N^{-4})$, each vertex appears in at most $5\log N$ sets in $\sset$, and $|\sset|\le 5r\log N$.
\end{observation}

We say that the event $\event$ happens iff either there exists a vertex that appears in more than $5\log N$ sets in $\sset$ or $|\sset|> 5r\log N$. It can be proved in the same way as \Cref{obs: bad event} that $\Pr[\event]=O(N^{-4})$.

We construct a collection $\sset'$ based on $\sset$ as follows. For each $v\in V$, if the sets in $\sset$ that contain $v$ are $S_1,\ldots,S_t$, then we independently pick an integer $i$ uniformly at random from $[t]$, and delete vertex $v$ from all sets $S_1,\ldots,S_{i-1}, S_{i+1},\ldots,S_t$. Let $\sset'$ be the obtain collection of sets after processing all vertices in $V$ in this way. Since for each set $S$ in $\sset$, $|E(S)|\le h$, from the construction of $\sset'$, the sets in $\sset'$ are disjoint and also satisfying that for each set $S'$ in $\sset'$, $|E(S')|\le h$. Moreover, if event $\event$ does not happen, then
\[
\expect{ |E(\sset')| }\ge 
\sum_{(u,v)\in E(\sset)}\Pr\Big[u,v\text{ belong to the same set in }\sset\Big]
\ge 
\sum_{(u,v)\in E(\sset)}\frac{1}{(5\log N)^2}
\ge \Omega\bigg(\frac{|E(\sset)|}{\log^2 N}\bigg).
\]

However, $\sset'$ may contain up to $(5r\log N)$ sets. We let $\sset''$ contain $r$ sets in $\sset'$ that contribute most edges in $E(\sset')$, so $|E(\sset'')|\ge \Omega(|E(\sset')|/\log N)$.
On the other hand, note that
\[\begin{split}
\expect{ |E(\sset)| }= & \text{ }
\Pr[\overline{\event}]\cdot
\expect{ |E(\sset)| \text{ }\Big| \text{ } \overline{\event}}
+
\Pr[\event]\cdot
\expect{ |E(\sset)| \text{ }\Big| \text{ } \event}\\
\le & \text{ }
\Pr[\overline{\event}]\cdot
\expect{|E(\sset)| \text{ }\Big| \text{ } \overline{\event}}
+
O\bigg(\frac{1}{N^4}\bigg)\cdot
N^2.
\end{split}
\]
Recall that $\expect{|E(\sset)|}\ge\Omega(\optwgp(G,r,h)/(\alpha(N^2)\log^2 N))$.
Combined with the above inequality and the fact that $\alpha(N^2)=o(N^2)$, we get that
$\expect{ |E(\sset)| \mid \overline\event}\ge \Omega(\optwgp(G,r,h)/(\alpha(N^2)\log^2 N))$. 
Therefore, 
%Via same arguments in \Cref{sec: DkC and WGP to DkS}, we can show that
\[\expect{|E(\sset'')|\mid \overline\event}\ge
\Omega\bigg(\frac{\expect{|E(\sset')|\mid \overline\event}}{\log N}\bigg)
\ge 
\Omega\bigg(\frac{\expect{|E(\sset)|\mid \overline\event}}{\log^3 N}\bigg)
\ge
\Omega\bigg(\frac{\optcl(G,k)}{\alpha(N^2)\log^5 N}\bigg).\] 

Since $|E(\sset'')| \le \optwgp(G,r,h)$ always holds, we then get that, with probability $1/(\alpha(N^2)\log^2 N)-O(1/N^4)\ge \Omega(1/(\alpha(N^2)\log^2 N))$,
$|E(\sset'')| \ge
\Omega\Big(\optwgp(G,r,h)/(\alpha(N^2)\log^5 N)\Big)$.

We finally augment sets in $\sset''$ by empty sets until $|\sset''|=r$, and return the resulting collection $\sset''$. This completes the description of the algorithm. Therefore, with probability $\Omega(1/(\alpha(N^2)\log^2 N))$,
$|E(\sset'')| \ge
\Omega\Big(\optwgp(G,r,h)/(\alpha(N^2)\log^5 N)\Big)$.

We repeat the whole algorithm $N^3$ times and output the best solution among all $N^3$ runs.
Since $\alpha(N^2)=o(N^2)$, with probability $1-2^{-\Omega(N)}$, the final output is an $O(\alpha(N^2)\log^5 N)$-approximation of instance $\optwgp(G,r,h)$.







\iffalse
\subsection{Proof of \Cref{lem: bipartite_WGP}}
\label{apd: Proof of bipartite_WGP}




Let $\alg$ be an efficient $\alpha(n)$-approximation algorithm for \WGP on bipartite graphs. We now construct an $O(\alpha(n))$-approximation algorithms for \WGP as follows. 
Let $\pwgp(G,r,h)$ be the input instance where $G=(V,E)$. We define graph $H=(V^1,V^2,E')$ as follows: $V^1=\set{v^1\mid v\in V}$, $V^2=\set{v^2\mid v\in V}$, and $E'=\set{(v^1,u^2), (v^2,u^1)\mid (v,u)\in E}$.
Consider now the instance $\pwgp(H,r,2h)$. We apply the algorithm $\alg$ to it, and let $\hset$ be the solution we get. Since $\alg$ is an $\alpha(n)$-approximation algorithm, $|E_H(\hset)|\ge \optwgp(H,r,2h)/\alpha(n)$. 

On the one hand, we show that $\optwgp(H,r,2h)\ge 2\cdot \optwgp(G,r,h)$. Let $\gset'$ be any solution of instance $\pwgp(G,r,h)$. We can construct a solution $\hset'$ to instance $\pwgp(H,r,2h)$ as follows. For each graph $G_i=(V_i,E_i)\in \gset'$, we define graph $H_i=\set{(v^1,u^2), (v^2,u^1)\mid (v,u)\in E_i}$ that is a subgraph of $H$. We then let $\hset'=\set{H_i\mid G_i\in \gset'}$. Clearly, for each $G_i\in \gset'$, $|E(H_i)|=2|E(G_i)|\le 2h$. Therefore, $\hset'$ is a feasible solution to instance $\pwgp(H,r,2h)$ and $|E(\hset')|\ge 2|E(\gset)|$, and so $\optwgp(H,r,2h)\ge 2\cdot \optwgp(G,r,h)$.

On the other hand, we can construct a solution $\gset$ to instance $\pwgp(G,r,h)$ using the solution $\hset$, such that $\expect{|E(\gset)|}\ge \Omega(\optwgp(H,r,2h)/\alpha(n))$.

We first construct a collection $\sset$ of vertex subsets of $V$ that contains, for each graph $H_i\in \hset$, a set $S_i\subseteq V$ constructed as follows.
For each vertex $v\in V$: 
\begin{itemize}
	\item if both $v^1, v^2$ belong to the same graph $H_i\in \hset$, then we add $v$ to $S_{i}$; 
	\item if $v^1\in H_1$ and $v^2\in H_2$ (where $H_1, H_2$ are distinct graphs in $\hset$), then we add $v$ to $S_{1}$ (the set in $\sset$ corresponding to $H_1$) with probability $1/2$ and add $v$ to $S_{2}$ (the set in $\sset$ corresponding to $H_2$) with probability $1/2$.
\end{itemize}

For each $S_i\in \sset$, we define graph $\tilde G_i$ on  $S_i$ where $E(\tilde G_i)=\set{(u,v)\mid u,v\in S_i,\text{ and }(u^1,v^2)\in E(H_i)}$, so $|E(\tilde G_i)|\le |E(H_i)|=2h$.
Moreover, for each edge $(u^1,v^2)\in E(\hset)$, it is easy to verify from the construction of $\sset$ that the probability that edge $(u,v)$ appears in some graph $\tilde G_i$ is at least $1/4$. Therefore,
\[
\expect{ \sum_{1\le i\le r}|E(\tilde G_i)| }\ge 
\sum_{u,v\in V}\mathbf{1}\Big[(u^1,v^2)\in E(\hset)\text{ or }(u^2,v^1)\in E(\hset)\Big]\cdot \frac 1 4
\ge \frac{|E(\hset)|}{2}\cdot \frac 1 4=\frac{|E(\hset)|}{8}.
\]
For each graph $\tilde G_i$, if $|E(\tilde G_i)|>h$, then we delete edges from it until it contains exactly $h$ edges. We denote the new graph by $G_i$ and let $\gset$ be the set of all graphs $G_i$. Since $|E(\tilde G_i)|\le 2h$, we have deleted at most half of the edges in $\bigcup_{1\le i\le r}E(\tilde G_i)$. Therefore, $\expect{ |E(\gset)| }\ge |E(\hset)|/16$, and so 
\[
\expect{ |E(\gset)| }\ge \Omega\bigg(\frac{|E(\hset)|}{16}\bigg)\ge \Omega\bigg(\frac{\optwgp(H,r,2h)}{\alpha(n)}\bigg).
\]
Altogether, $\expect{ |E(\gset)|}=\Omega(\optwgp(G,r,h)/\alpha(n))$.
Therefore, our algorithm returns an $O(\alpha(n))$-approximate solution to instance $\pwgp(G,r,h)$.

\fi


==> lemma-proof.tex <==

\newpage
\subsection{Proof of \Cref{lem: WGP_BCS}}
\label{sec: Proof of lem: WGP_BCS}



\iffalse
\begin{lemma}
	\label{lem: WGP_BCS}
	There is an efficient algorithm, whose input consists of an instance $\pcn(G,L)$ of the \BCS problem with $|V(G)|=N$, and a solution $H$ to this instance, with  $|E(H)|\ge 4N\log^6N$. The algorithm computes integers $r,h>0$, such that $r\cdot h^2\le L\cdot \log^6N$ and $r\cdot h\ge \Omega(|E(H)|/ \log N)$ hold, together with a good solution $\set{H_1,\ldots,H_r}$ to instance $\pwgp(G,r,h)$ of \WGP.
\end{lemma}
\fi



Let $\hat G$ be any graph. A \emph{cut} in $\hat G$ is a partition $(A,B)$ of vertics of $\hat G$ into two non-empty subsets. The \emph{value} of the cut $(A,B)$ is $|E(A,B)|$. For a parameter $1/2<\beta<1$, we say that cut $(A,B)$ is \emph{$\beta$-balanced}, if $|E(A)|,|E(B)|\le \beta\cdot |E(\hat G)|$. We say that cut $(A,B)$ is a \emph{minimum $\beta$-balanced cut} if it is a $\beta$-balanced cut whose value is the smallest among all such cuts.  We use the following theorem that follows from \cite{ARV}.

\begin{theorem}
\label{thm: bal_cut alg}
There is an efficient algorithm, that, given a graph $\hat G$ with $|V(\hat G)|=N$, computes a $(4/5)$-balanced cut in $G$, whose value is at most $O(\sqrt{\log N})$ times the value of the minimum $(3/4)$-balanced cut in $\hat G$.
\end{theorem}

We use the following theorem, that is a simple corollary of the Planar Separator Theorem by Lipton and Tarjan \cite{planar-separator}, and was formally proved in  \cite{chuzhoy2022subpolynomial}\mynote{please update in bibliography to STOC version and list pointer to arxiv version as a note.}. A variation of this theorem for vertex-balanced cuts was proved in \cite{pach1996applications}. 

\begin{theorem}[Lemma 4.12 in the full version of \cite{chuzhoy2022subpolynomial}]
\label{thm: bal_cut size}
Let $\hat G$ be a connected graph with $m$ edges and maximum vertex degree $\Delta<\frac{m}{2^{40}}$. If $\CrN(\hat G)\le \frac{m^2}{2^{40}}$, then the value of the minimum $(3/4)$-balanced cut in $\hat G$ is at most $O(\sqrt{\CrN(\hat G)+\Delta\cdot m})$.
\end{theorem}

We now provide the proof of \Cref{lem: WGP_BCS}. Recall that we are given an instance $\pcn(G,L)$  of \BCS, where $|V(G)|=N$, together with a solution $H$ to this instance, such that  $|E(H)|\ge 4N\log^6 N$. 

The algorithm iteratively decomposes graph $H$, as follows.  Throughout the algorithm, we maintain a collection $\hset$ of connected subgraphs of $H$, that are all mutually disjoint. Each graph $H'\in \hset$ is marked as either \emph{active} or \emph{inactive}. At the beginning of the algorithm, we set $\hset=\set{H}$, and we mark graph $H$ as active. The algorithm performs iterations, as long as at least one graph in $\hset$ is inactive. 

In order to execute an iteration, we select an arbitrary active graph $H'\in \hset$. We apply the algorithm from \Cref{thm: bal_cut alg} to compute a $(4/5)$-balanced cut $(A,B)$ of $H'$. If $|E_{H'}(A,B)|\ge \frac{|E(H')|}{\log^2 N}$, then we mark $H'$ inactive and continue to the next iteration. Otherwise, we remove graph $H'$ from $\hset$, and we add all connected components of graphs $H'[A]$ and $H'[B]$ to $\hset'$, that are all marked as active graph. We then continue to the next iteration. This completes the description of the algorithm. Let $\hset'$ be the collection $\hset$ of subgraphs of $H$ that we obtain at the end of the algorithm. We prove the following observation.

\begin{observation}
$\sum_{H'\in \hset'}|E(H')|\ge |E(H)|/2$.
\end{observation}
\begin{proof}
We prove the observation via a charging scheme as follows. Whenever some graph $H'$ is replaced by graphs $H'[A]$ and $H[B']$, we charge the edges in $E_{H'}(A,B)$ to all remaining edges in $H'[A]$ and $H[B']$, so each edge is charged at most $O(1/\log^2 N)$. Observe that every time an edge is charged, the number of edges in the graph in $\hset$ that the edge belongs to decreases by at least a factor of $(4/5)$, so every edge is charged at most $O(\log N)$ times. Therefore, the total charge on all edges is at most $O(\log N)\cdot O(1/\log^2 N)<1/2$. The observation now follows.
\end{proof}

Consider now the final collection $\hset'$ of graphs. We say that a graph $H'\in \hset'$ is \emph{dense} iff $|E(H')|\ge |V(H')|\cdot \log^6 N$; otherwise we say it is \emph{sparse}. Observe that the total number of edges in all dense graphs in $\hset'$ is at least $ |E(H)|/4\ge N\log^6 N$, since otherwise 
\[
|E(H)|\le 4\cdot \sum_{H\in \hset':\text{ sparse}} |E(H)|
< 4\cdot \log^6 N\cdot\sum_{H\in \hset':\text{ sparse}} |V(H)|\le 4N\cdot \log^6 N,
\]
a contradiction to the assumption that $|E(H)|\ge 4N\cdot \log^6 N$. 

Consider now any dense graph $H'\in \hset$. Since it is marked inactive by the algorithm, the $(4/5)$-balanced cut of $H'$ computed by the algorithm from \Cref{thm: bal_cut alg} has value at least $|E(H')|/\log^2 N$, and therefore the minimum $(3/4)$-balanced cut of $H'$ has value at least $\Omega(|E(H')|/\log^{2.5} N)$. 
On the other hand, since $H'$ is a dense graph, the maximum degree $\Delta$ of $H'$ is at most $|V(H')|\le |E(H')|/\log^6 N$, which is less than $|E(H')|/2^{40}$.  Therefore, from \Cref{thm: bal_cut size}, we get that either $\CrN(H')\ge |E(H')|^2/2^{40}$ holds, or $\sqrt{\CrN(H')+\Delta\cdot |E(H')|}=\Omega(|E(H')|/\log^{2.5} N)$ holds. In either case, we get that $\CrN(H')=\Omega(|E(H')|^2/\log^{5} N)$.

Let $\hset''$ be the set of all dense subgraphs in $\hset'$.
We now apply the algorithm from \Cref{obs: equal_size} to the set $\hset''$ of graphs, and let $\hset'''$ be the collection we obtained. Define $r=|\hset'''|$ and let $h$ be such that $h/2\le |E(H')|\le h$ for all $H'\in \hset'''$. We output $r,h$ and $\hset'''$.

Since $H$ is a subgraph of $G$, it is easy to verify that $\hset'''$ is a good solution to instance $\pwgp(G,r,h)$. From the construction of $r,h,\hset'''$, \[rh=\Omega(|E(\hset''')|)=\Omega(|E(\hset'')|/\log N)=\Omega(|E(\hset')|/\log N)=\Omega(|E(H)|/\log N).\]
Finally, since for each graph $H'\in \hset'''$, $\CrN(H')=\Omega(|E(H')|^2/\log^{5} N)$, we get that
\[r\cdot h^2\le \sum_{H'\in \hset'''}4\cdot |E(H')|^2
\le \sum_{H'\in \hset'''}O(\log^{5} N)\cdot \CrN(H')
\le O(\log^5 N)\cdot \CrN(H)\le L\cdot \log^6 N.
\]

